Recruiting credible participants for field studies in software engineering research

Context: Software practitioners are a primary provider of information for field studies in software engineering. Research typically recruits practitioners through some kind of sampling. But sampling may not in itself recruit credible participants. Objectives: To propose and demonstrate a framework for recruiting professional practitioners as credible participants in field studies of software engineering. Method: We review existing guidelines, checklists and other advisory sources on recruiting participants for field studies. We develop a framework, partly based on our prior research and on the research of others. We search for and select three exemplar studies (a case study, an interview study and a survey study) and use those to demonstrate the application of the framework. Results: Whilst existing guidelines etc. recognise the importance of recruiting participants, there is limited guidance on how to recruit the right participants. Our demonstration of the framework with three exemplars shows that at least some members of the research community are aware of the need to carefully recruit participants. Conclusions: The framework provides a new perspective for thinking about the recruitment of credible practitioners for field studies of software engineering. In particular, the framework identifies a number of characteristics not explicitly addressed by existing guidelines.

==> x_archive/Old_illustrative_examples.tex <==
\section{Illustrative examples}
\label{section:illustrative-examples}

We discuss two papers as illustrative examples of the issues we explore. These two papers are selected because of the  level of detailed explanation reported in the respective papers. The first paper, by Karlstr{\"o}m and Runeson \cite{karlstrom2006integrating}, presents a case study. The second paper, by Schermann et al. \cite{SCHERMANN201841}, presents two interview studies and a survey study. 

\subsection{The transformation of information}
\label{subsection:reference-example}

Karlstr{\"o}m and Runeson \cite{karlstrom2006integrating} present a study of two large, independent software projects that use eXtreme Programming within a stage--gate project management model. Our interest in their study is in the way that they reason about the research process.  

Karlstr{\"o}m and Runeson present a model of the information used in their study and of the transformation of that information. For convenience, Karlstr{\"o}m and Runeson’s model of information--transformation is reproduced here in Figure \ref{figure:karlstrom-and-runeson-figure}. The two projects the studies are identified as EMW and ABB.

The \textit{source} of information about the items of interest -- the two cases, EMW and ABB -- comes from the subjects' perceptions of the two items. (Strictly speaking, a case study would rely on other sources of information as well, such as project documents. Given the focus of our paper, we concentrate on participants of the study.)

Karlstr{\"o}m and Runeson \cite{karlstrom2006integrating} discuss threats to the validity of the research that arise as the information is transformed. They also discuss strategies for dealing with those threats. Our paper focuses on the lowest three levels of their model but also generalises those three levels beyond case study research. We also re-label the model. We present our more generalised version in Figure \ref{figure:generalised-karlstrom-and-runeson-figure}.

\begin{figure}
    \centering
    \includegraphics[scale=0.8]{images/karlstrom_and_runeson_figure.png}
    \caption{Karlstr{\"o}m and Runeson \cite{karlstrom2006integrating} levels and transformation of information in their research process}
    \label{figure:karlstrom-and-runeson-figure}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale=0.4]{images/generalised_karlstrom_and_runeson_figure_v1.png}
    \caption{Generalised version of the lower three levels of Karlstr{\"o}m and Runeson's \cite{karlstrom2006integrating} research process. \textcolor{magenta}{Rework as a table?}}
    \label{figure:generalised-karlstrom-and-runeson-figure}
\end{figure}

Many of the threats and strategies discussed by Karlstr{\"o}m and Runeson \cite{karlstrom2006integrating} relate to higher levels of their model, and therefore are not relevant for our discussion. Also, the threats and strategies that Karlstr{\"o}m and Runeson \cite{karlstrom2006integrating} do identify for the lower levels are different to those we identify. For these reasons, we do not reproduce their tables of threats and strategies here.

Because Karlstr{\"o}m and Runeson \cite{karlstrom2006integrating} study two cases participants are therefore recruited in relation to specific, identifiable situations in the world. A consequence is that the information that the participants are asked for is also, at least in principle, constrained. Furthermore, Karlstr{\"o}m and Runeson also interview the participants, providing the opportunity (again at least in principle) to clarify, challenge etc. the information provided by those participants. In order words, the researchers know (or can know) something about the nature of the transformations between levels of information (at TA and TB, in Figure \ref{figure:generalised-karlstrom-and-runeson-figure}), and something about the information--selection decisions being made at levels 1, 2 and 3.

In interview studies, the situation can be much more varied and therefore different to the Karlstr{\"o}m and Runeson \cite{karlstrom2006integrating} study. The researcher may have less influence or control on the participants recruited, e.g. using a convenience sample. Because the interview allows for interaction, the researcher may know something about the nature of transformations, may be able to influence those transformations (e.g., to challenge answers), and may be able to know and constrain something about the information-selection occurring at levels 1, 2 and 3.

In surveys the situation is typically very different. The researchers have little, if any, influence or control on the situations in the world to which the participants refer. They also have little opportunity to influence the information provided by the participants. In order words, the researchers knows little about the nature of transformations TA and of TB, or about the information--selection at level 1 and 2.

\subsection{Interviews and survey}

Schermann et al. \cite{SCHERMANN201841} report a multi--method empirical study on continuous experimentation in software development companies. Their multi--method study comprises two interview studies and a survey study. The paper is valuable as an illustrative example for several reasons: they explain the overall research methodology; they explain the participant recruitment and sample for each study; they discuss threats to validity for each study; they provide a detailed appendix with further information on the design and conduct of the studies; and, finally, they complement the published paper with an online supplement. For simplicity we focus here on their first interview study and their survey study (our discussion of their first interview study we essentially be repeated for their second interview study). These two studies are summarised in Table \ref{table:multi-method-illustrative-example}. 

The research questions for their multi--method study were:
\begin{itemize}
    \item RQ1 : What principles and practices enable and hinder organizations to leverage continuous experimentation?
    \item RQ2 : What are the different flavors of continuous experimentation and how do they differ?
\end{itemize}


\subsubsection{First interview study}

In their discussion of the threats to the first interview study, Schermann et al. write, ``\dots a potential threat to our empirical findings is that our results are not generalizable beyond the subjects involved\dots'' (\cite{SCHERMANN201841}, p. 46). Elsewhere, also in relation to the first interview study, the paper says, ``Snowball sampling helped us to increase our sample size'' (\cite{SCHERMANN201841}, p. 46). Given the two research questions, that the multi--method study is focused on experimentation in software development, and the different types of case (i.e., individual, process, team, company; see Table \ref{table:multi-method-illustrative-example}), it is not clear why generalisation would be on the basis of \textit{participants}.

To be fair, Schermann et al. \cite{SCHERMANN201841} recognise there is a threat to generalisability. Their mitigation of that threat is through the mixed--method approach: ``We mitigate this effect by employing a mixed--method study validating our interview findings in a more general context using a quantitative survey in the following step.'' (\cite{SCHERMANN201841}, p. 46).

We suggest that the 20 participants might better be understood as a kind of \textit{sampling frame} (cf. the discussion of sampling in Section \ref{subsection:sampling}) through which a sample of real--world phenomena are indirectly studied. The difficulty is that it remains unclear what `units' of phenomena are being studied `through' these participants. Or in other words, what is the case from which one seeks to generalise (either analytically or statistically)?

\begin{table}[!ht]
    \small
    \caption{Summary of Schermann et al.'s multi--method study \cite{SCHERMANN201841}}
    \label{table:multi-method-illustrative-example}
    \centering
    \begin{tabular}{| p{1.5cm} | p{5.7cm} | }
        \hline
        \textbf{Dimension} & \textbf{Description}\\
        \hline
        \hline
        \multicolumn{2}{|l|}{First interview study}\\
        \hline
        Recruitment process & From industry partners, personal networks and snowballing.\\
        \hline
        Sample & ``to recruit interview participants that are approximately evenly distributed between organizations of varying sizes, divergent domains, and backgrounds (years of experience and age of participants)'' (p. 46)\\
        \cline{2-2}
        & 20 participants: Software Engineer, DevOps Engineer, Solution Architect, Public Cloud Architect, Program Manager, Project Lead, Director of Engineering\\
        \cline{2-2}
        & 3 company types: Startup, SME, Corporate\\
        \cline{2-2}
        & 4 applications types: Web, Enterprise, Desltop, Embedded\\
        \cline{2-2}
        & \textcolor{magenta}{X application domains: \dots}\\
        \cline{2-2}
        & 6 countries: Austria, Germany, Switzerland, Ireland, Ukraine, \& the US.\\
        \hline
        Case/s & 4 types: Individual, process, team, company\\
        \hline
        Data \mbox{collection} & Topics followed the natural flow of the interview.\\
        \cline{2-2}
        & Not all questions were asked of all participants.\\
        \hline
        Threats & ``\dots we rely on self--reported (as opposed to observed) behavior and practices (self--reporting bias).'' (p. 46)\\
 
        \hline     
        \hline
        \multicolumn{2}{|l|}{Survey study}\\
        \hline
        Recruitment process & distributed the survey within  personal networks, social media, via two DevOps related newsletters, and via a German-speaking IT news portal.\\
        \hline
        Sample & 187 respondents\\
        \cline{2-2}
        & Experience: 8yrs average (4yrs SD)\\
        \hline
        Case/s & Similar to the interviews, some questions focused on the development and deployment process on the team or company level\\
        \cline{2-2}
        & 3 company types: Startup, SME, Corporate\\
        \cline{2-2}
        & 6 application types: Embedded, Mobile, Desktop, Enterprise, Web, Other\\
        \hline
        Threats & it is likely that the survey has attracted a respondent demography with substantial interest and familiarity with continuous deployment and experimentation practices (self--selection bias).\\
        \cline{2-2}
        & participants may have provided idealized data about their companies’ states on CD and experimentation (self--reporting bias).\\
        
        % \hline
        % \hline
        % \multicolumn{2}{|l|}{Second study}\\
        % Participant recruitment & \\
        % Sample & 11 participants: Software Engineer, DevOps Engineer, Head of Department, Team Lead, Head Release Engineering, Director of Engineering\\
        % & 3 company types: Startup, SME, Corporate\\
        % & 1 applications type: Web\\
        % & X application domains: \dots\\
        % & 4 countries: Germany, Ukraine, UK, \& the US.\\
        % Case/s & \\ 
        
        \hline
    \end{tabular}
\end{table}

\subsubsection{Survey study}

In the appendix to their paper, Schermann et al. \cite{SCHERMANN201841} write, ``\dots in surveys subjects are sampled from a population to which results are intended to be generalized.'' (\cite{SCHERMANN201841}, p. 55). As with the first interview study, it is not clear whether participants are the appropriate \textit{population} from which to sample items (i.e., participants). 

\subsection{Summary}

\textcolor{magenta}{To be written.}

==> x_archive/X5_old_framework.tex <==
\section{OLD Framework}
%\label{section:framework-and-checklist}

In this section we present and discuss the framework for recruiting credible practitioners. The framework comprises: a simple research model for reference; the identification of participant roles, together with the mapping of these roles to Falessi et al.'s~\cite{falessi2018empirical} R\textsuperscript{3} model; the identification of five characteristics that influence the quality of information a participant can provide; a  discussion of the importance of demographics; a discussion of three well--accepted research strategies for collecting information from participants (i.e., the case study, interview study and survey) together with a comparison of those strategies; a discussion of further issues that should be considered; and, finally, a discussion of the contribution of the framework to the recruitment of credible practitioners.

We complement the framework with a checklist, presented in Appendix A. The checklist provides a set of questions, derived from the framework, to `ask' of actual empirical studies, irrespective of whether these studies are in preparation, in conduct, or completed. 

\subsection{\textcolor{magenta}{A reference model for the research process}}

Figure \ref{figure:research-model} presents a simple model of the research process for empirical software engineering. The model is intended to be used as a reference for the subsequent discussion. In the model, a theory of some kind provides the grounds for a proposition. The proposition is studied empirically. Taking the natural sciences as an example, the empirical world can be studied directly. For empirical software engineering research, many aspects of software engineering practice can be studied directly (e.g., source code), however many other aspects of software engineering practice can only be studied indirectly, i.e., through engaging with software practitioners who themselves interact with the empirical world of software engineering. This is the focus of the reference model. In the model, practitioners provide information about the empirical world. This information is broadly of two types: facts that describe some aspect of the world, and beliefs about the world.

As already noted, the reference model is a simplification. For example, grounded theories are generated bottom--up from the empirical world. As another example, the propositions of the model may be hypotheses, research questions, or other kinds of testable or otherwise investigatable statements.

\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.5]{images/research_model.png}
    \caption{A simple reference model of the research process for empirical software engineering research}
    \label{figure:research-model}
\end{figure}

Again for simplicity, we assume that theories are constructed from four fundamental constructs: the \emph{actor}, the \emph{technology}, the \emph{activity} and the \emph{software artefact}. These constructs are well--accepted in software engineering research~\cite{sjoberg2008building}. These constructs exist within a \emph{context} \cite{petersen2009context, dybaa2012works, clarke2012situational} which, by its nature, is difficult to define.

The scope of the theory, and therefore of the propositions, will align in some way with the empirical world being studied. For example, a researcher working with a theory and propositions about requirements engineering is unlikely to be empirically investigating actual code inspections. Furthermore, the researcher will empirically study attributes of the four constructs as they relate to requirements engineering, e.g., requirements engineers (\emph{actor}), who use templates (\emph{technology}), to elicit (\emph{activity}) requirements (\emph{software artefact}); as well as \emph{context}, of course.

In Figure \ref{figure:research-model}, the participants are expected to be drawn from the empirical world as that world aligns with the theory and propositions. Remaining with our earlier example, for the researcher studying requirements engineering, the researcher would conduct empirical studies with requirements engineers, or similar, as the participants, and ask those requirements engineers about requirements engineering. 

\subsection{\textcolor{magenta}{NEW: Participants as a sampling frame}}
\austen{What is new here is simply the insertion of a subsection heading}

In the related work in Section~\ref{subsection:sampling}, we discussed the sampling of items from a population of interest, or alternatively sampling items from a sampling frame. In software engineering research, it seems to be common to seek a sample of participants that is in some way representative of the population of practitioners. In other words, it often seems to be the case that researchers define populations in terms of practitioners. Our reference model in Figure \ref{figure:research-model} allows for other kinds of items of interest.

We suggest that, depending on the theory and propositions, it may be more effective to treat participants as a kind of sampling frame through which the items of interest from the empirical world are sampled, and therefore indirectly studied. Our suggestion is illustrated in Figure \ref{figure:participants-as-a-sampling-frame}.

\begin{figure}
    \centering
    \includegraphics[scale=0.4]{images/participants-as-sampling-frame-v2.png}
    \caption{Participants as a sampling frame. Each participant has access to one or more items of interest from the population, and the aggregate of participants provides a sampling frame.}
    \label{figure:participants-as-a-sampling-frame}
\end{figure}

Remaining with our earlier example, if the researcher intends to study the \emph{attitude} of requirements engineers then it makes sense to treat requirements engineers as the population and to sample from that population. This is because attitude is a property, or attribute, of the requirements engineers themselves. But if the researcher intends to study any one or more of the other three constructs in theories -- i.e., \emph{activity}, \emph{technology} or \emph{artefact}, or \emph{actors} other than the participant -- then the population of interest is not the requirements engineer but rather one or more of these other constructs. More strictly, the population of interest is likely to be a configuration of \emph{actor}, \emph{activity}, \emph{technology} and \emph{artefact}, all within one or more contexts. The researcher should therefore sample from across all of the appropriate constructs of interest. The implication is that participants should be recruited for the `access' they give to the population of actor, activity, technology and artefact, and not sampled for their representativeness of practitioners. In other words, a participant should be recruited for the contribution they can make to the formation of a sampling frame for sampling the items of actual interest. Recruiting participants in this way helps to ensure that the researcher collects information (either facts about the world, or beliefs about the world) that are drawn in relation to the items of interest.

Participants will often be software practitioners who are located somewhere \emph{within} a software engineering situation and can therefore observe other \emph{actors}, as well as the \emph{activities}, \emph{technologies} and \emph{artefacts} of the situation. Sometimes a participant may be a software practitioner who is located outside of the situation but who can, for some reason, contribute to the formation of a sampling frame.

% \subsection{Characteristics of participants}

\subsection{Participant roles}
\label{subsubsection:roles}

In Section~\ref{subsection:Rmodel}, we discussed Falessi et al.'s~\cite{falessi2018empirical} R\textsuperscript{3} model comprising three elements, i.e., Real, Relevant, and Recent. Accepting that a practitioner satisfies these three characteristics, there is a further set of characteristics that concern the \emph{role} of the practitioner. We define three roles here (specific studies may need to define additional roles for the respective study, or an alternative set of roles):
\begin{itemize}
    \item The practitioner who is a \emph{Performer} within the situation.
    \item The practitioner who is an \emph{Observer}, but not a \emph{performer}, and is located elsewhere within the situation.
    \item The practitioner who is an \emph{Advisor} with sufficient experience of other situations for the advisor's experience to have value to the research. The more experienced, and the more widely experienced, a software practitioner becomes the more likely they will have \emph{some} real experience of relevance to the research (though, as we recognised, some of that experience may not be recent).
    % The role of \emph{advisor} relates to our earlier identification of the `outside practitioner'.
\end{itemize}

In reality, some of the practitioner's experience may allow that practitioner to be classified as an \emph{Performer}, whilst some other of the same practitioner's experience may allow that practitioner to be classified as an \emph{Observer}, and yet some other of the same practitioner's experience may allow that practitioner to be classified as an \emph{Advisor}; and indeed some of the practitioner's experience may not allow classification according to the three roles, e.g., because that experience is not relevant. We acknowledge this complication; it is a complication inherent within software development and research into software development.

Our suggestion is that the researcher evaluates a practitioner against these three roles in the order that we have presented them, i.e., first determine whether the practitioner could be treated as a \emph{Performer}. According to our framework, a practitioner who could not satisfy any of the three roles would in principle be rejected as a participant. In practice, the researcher may introduce an additional role or roles for practitioners, where it is appropriate to do so for their research.

Table~\ref{table:participant-characteristics} maps the roles to the three elements of Falessi et al.'s~\cite{falessi2018empirical} R\textsuperscript{3} model.

\begin{table*}[htp]
    \small
    \caption{Summary of participant characteristics}
    \label{table:participant-characteristics}
    \centering
    \begin{tabular}{| p{2.8cm} | c | c | c | }
        \toprule
        \textbf{Role} & \textbf{Real} & \textbf{Relevant} & \textbf{Recent}\\
        \midrule
        Performer & YES & YES & YES\\
        Observer & YES & yes & yes \\
        Advisor & yes & maybe & maybe \\
        \bottomrule
        \multicolumn{4}{p{9cm}}{Notes:}\\
        \multicolumn{4}{p{9cm}}{YES=strongly meets criterion.}\\
        \multicolumn{4}{p{9cm}}{yes=moderately meets criterion.}\\
        \multicolumn{4}{p{9cm}}{maybe=may meet criterion depending on context.}\\
    \end{tabular}
\end{table*}

\subsection{Characteristics of practitioners affecting the quality of their information}
\label{sec:characteristics}

In addition to role and to Falessi et al.'s~\cite{falessi2018empirical} three Rs, we suggest five further characteristics of the practitioner that might affect the quality of information they can provide as a participant in a study. These characteristics are partly derived from Marshall's~\cite{marshall1996key} five characteristics of a key informant, summarised in Table \ref{table:key-informants} in Section \ref{section:key-informants}. First, the practitioner must have the willingness or, alternatively phrased, the motivation to openly share information. Second, and in general, the greater the quantity of situations experienced by the practitioner, the more experienced is the practitioner for the research. Third, the more the practitioner is able to \emph{carefully} observe events and, through that careful observation, to help prevent or reduce bias in their observation, the more valuable is the practitioner for the research. Fourth, the more the practitioner is able to subsequently \emph{reflect} on those observations as they develop their experience and, through that reflection, to help prevent or reduce biases in the information they share with the researchers, the more valuable is the practitioner for the research. Fifth, and finally, the more the practitioner can distinguish between the situations and so provide only the more valid and relevant information to the researcher, the more valuable is the practitioner for the research. For the last characteristic, it may be more valuable to the researcher for the practitioner to \emph{restrict} the information they share to a specific situation, or situations, to ensure the information is more valid and more relevant, cf. the role of the sampling frame.
% And it is, of course, a responsibility of the researcher to support the informant in that recruitment process.

These five characteristics -- of willingness, of quantity of experience, of observational ability, of reflective ability, and of situation selection -- are all simplifications, and are all very challenging to measure. Again, the principle here is that we seek to recruit participants who are able to provide more valid and more relevant information to the research. 

\subsection{Demographics of participants}

Empirical studies of software engineering often report the demographics of the participants. For example, in one of their survey studies of professional software engineers at Microsoft, Begel and Zimmerman~\cite{begel2014analyze} found statistically significant differences in responses to 29 questions, based on the demographics of the respondents. And taking one pervasive demographic -- gender -- as a another example, Carver and Serebrenik~\cite{carver2019} summarise several papers published in the 2019 edition of the International Conference on Software Engineering (ICSE) that discuss gender and software engineering.

These examples highlight the importance of considering demographics when collecting information from practitioners about their experience of software practice, i.e., practitioners with differing demographics may have differing experiences and may therefore provide different information. Also, it may be that the three roles we have identified have different demographic profiles, e.g., different proportions of gender or age for the different roles.

Because of the inherent nature of demographics, and because of the pervasiveness of collecting demographic information in software engineering research, we explicitly recognise demographics in our framework, rather than only implying it in the existing characteristics.

\subsection{Research strategies for collecting information from participants}

As noted earlier, and broadly speaking, researchers can collect two types of information from participants, i.e., facts about the world and beliefs about the world. Table \ref{table:types-of-information} maps the types of information that can be provided by the different roles. The table also recognises that the quality of this information can vary, depending on the five additional characteristics of participants, i.e., willingness (W), quantity of experience (E), observational ability (O), reflectiveness (R) and situation-selectivity (S), as well as demographics (D). The table indicates that the different roles can provide different types of information and, depending on the characteristics of the participant, different degrees of quality of information.  We intentionally do not populate the Quality criteria. 

\begin{table*}[htp]
    \small
    \caption{Types and quality of information the respective role can provide.}
    \label{table:types-of-information}
    \centering
    \begin{tabular}{| l | c | c || c | c | c | c | c | c | }
        \toprule
        & \multicolumn{2}{| c ||}{\textbf{Type}} & \multicolumn{6}{| c |}{\textbf{Quality}}\\
        \textbf{Role} & \textbf{Fact} & \textbf{Beliefs} & \textbf{W} & \textbf{E}  & \textbf{O} & \textbf{R} & \textbf{S} & \textbf{D}\\
        \midrule
        Performer & YES & YES & \multicolumn{6}{c |}{\dots} \\
        Observer & yes & yes & \multicolumn{6}{c |}{\dots} \\
        Advisor & -- & yes & \multicolumn{6}{c |}{\dots}\\
        \bottomrule
        \multicolumn{9}{l}{Notes:}\\
        \multicolumn{9}{l}{YES = more likely to provide}\\
        \multicolumn{9}{l}{yes = may be able to provide}\\
        \multicolumn{9}{l}{-- = cannot provide facts about the item/s of interest}\\
        \multicolumn{9}{l}{We intentionally do not populate the Quality criteria.}\\
    \end{tabular}
\end{table*}

In a case study, the researcher focuses on one (or sometimes more than one) specific situation in its natural environment and studies that situation intensively~\cite{runeson2009guidelines}. The researcher works with some kind of research model, however formally or informally developed, and makes inferences (e.g., inductively, abductively, or deductively) between the specific situation and the model. Because the researcher works with a specific situation, the researcher is much better able to identify practitioners that align with the research model, is better able to determine the suitable \emph{role} of the practitioner, is better able to assess the quality of information the practitioner might provide (cf. Table~\ref{table:types-of-information}), and can therefore better evaluate whether each practitioner is suitable as a credible participant. The researcher is also better able to control the types of information collected, i.e., to collect facts about the world or beliefs about the world, or both. Finally, the researcher is able to use methods of triangulation across multiple sources of information, e.g., across participants, project documentation, emails,to get a better `handle' on the situation and to better assure the validity and relevance of information in relation to the research model.

In an interview study, the researcher typically focuses on collecting information from multiple practitioners who each have experience of one or more situations. Again, the researcher works with some kind of research model etc. Because the researcher typically has direct contact with the prospective participants, as part of the recruitment process, the researcher has the opportunity to identify practitioners that align with the research model, is better able to determine the suitable \emph{role} of the practitioner, is better able to assess the quality of information the practitioner might provide (cf. Table~\ref{table:types-of-information}), and can therefore better evaluate whether each practitioner is suitable as a credible participant. The researcher is also better able to control the types of information collected, i.e., to collect facts about the world or beliefs about the world, or both. Unlike the case study, however, the researcher is less likely to be able to draw on triangulation as a approach to quality assurance of the information collected from the participants.

In a survey, the researcher typically focuses on collecting information from multiple practitioners who have experience of situations where those situations are, \emph{at best}, only partially known to the researcher. Again, the researcher works with some kind of research model etc. Because the researcher has limited control on the recruitment process, the researcher lacks the opportunity to identify practitioners that align with the research model, is not able to determine the suitable \emph{role} of the practitioner, is not able to assess the quality of information the practitioner might provide (cf. Table~\ref{table:types-of-information}), and therefore has limited opportunity to evaluate whether each practitioner is suitable as a credible participant. The researcher also has limited control on the types of information the participant provides, i.e., whether the participant reports facts about the world or beliefs, or both or neither. The researcher is also not able to draw on triangulation as a approach to quality assurance of the information collected from the participants.

There are several survey--study designs available to the researcher. For example, the researcher might ask the participant to respond to the survey on the basis of one specific situation that the participant has experienced, ask the participant to provide a description of the situation, or to ask several practitioners to provide information about the same situation (offering a kind of triangulation). With all these designs, there remain challenges in assuring the recruitment of appropriately credible participants.

Table \ref{table:compare-research-strategies-v04} provides a summary comparison of the three research strategies in relation to the framework.

\begin{table*}[htp]
    \small
    \caption{A comparison of research strategies in relation to components of the framework.}
    \label{table:compare-research-strategies-v04}
    \centering
    \begin{tabular}{| p{3.6cm} | c |  c | c | }
        \toprule
        \textbf{Property} & \textbf{Case Study} & \textbf{Interview Study} & \textbf{Survey Study}\\
        \midrule
        % \hline
        % \hline
        \multicolumn{4}{| l |}{\emph{Situations}}\\
        % \hline
        \midrule
        Explicitness of source situation/s & Explicit & Explicit & Implied \\
        % \hline
        \midrule
        Level of abstraction & Variable & Consistent & Unknown\\
        % \hline
        \midrule
        Number of situations studied & 1 or Few & Variable & Unknown \\
        % \hline
        \midrule
        \multicolumn{4}{| l |}{\emph{Participants}}\\
        \hline
        Direct access to candidates & Good & Good & Limited\\
        % \hline
        \midrule
        Number of participants & Some & Some to many & Many \\
        % \hline
        \midrule
        Number of participants per situation & Some & 1 or Some & 1  \\
        % \hline
        \midrule
        Ability to select practitioners & Easier & Easier & Harder \\
        % \hline
        \midrule
        Ability to evaluate practitioners & Easier & Easier & Harder\\
        % \hline
        \midrule
        Ability to control types of information & Easier & Easier & Harder \\
        % \hline
        \midrule
        \multicolumn{4}{|l|}{\emph{Types of information}}\\
        % \hline
        \midrule
        Restrict to description & Easier & Easier & Harder\\
        % \hline
        \midrule
        Restrict to belief & Easier & Easier & Harder\\
        % \hline
        \midrule
        \multicolumn{4}{|l|}{\emph{Inference to research model}}\\
        % \hline
        \midrule
        Focus of information validation & Within situation & Across responses & Across responses\\
        % \hline
        \midrule
        Method of information validation & Triangulation & Replication & Statistical\\ 
        % \hline
        \midrule
        Method of generalisation & Analytical & Analytical & Statistical\\
        \bottomrule
    \end{tabular}
\end{table*}

\subsection{Additional considerations}
\label{section:additional-considerations}

When applying the framework some additional considerations will need to be addressed. As one example, using some kind of key participant in research potentially reduces the number of participants and therefore increases the likelihood that the participant/s might be identifiable, e.g., when conducting an interview study in a company. This raises ethical issues. We do not consider these issues in this paper, however Strandberg~\cite{Strandberg2019}, for example, discusses ethical issues affecting interviews in software engineering. As a second example, \emph{finding} key participants may be challenging, particularly as the researcher becomes more selective on the characteristics of the participant. But, as we noted from Bernard et al.'s~\cite{bernard1984problem} work in Section~\ref{section:related-work}, collecting information from many inaccurate participants will not solve the accuracy/validity problem, and will, as a consequence, also not produce relevant findings.

\subsection{Contribution of the framework}
\austen{This needs reworking}

The framework is intended to encourage the researcher to think more carefully about the recruitment of credible participants for their empirical studies of software practice. Returning to our earlier example, a researcher may invite requirements engineers to participate in an empirical study. The framework encourages the researcher to consider whether and how the participant provides access to the empirical world, as well as the kinds of information the participant can provide. Not all requirements engineers can provide the kinds of access the researcher may want, and not all requirements engineers can provide the kinds of information the researcher may want. A requirements engineer (\emph{actor}) who is actively undertaking requirements engineering (\emph{activity}) using appropriate resources (\emph{technology}) and producing requirements specifications (\emph{artefacts}) that align with the theory and propositions of the research model is expected to have the most direct contact with the empirical world; in other words, may be understood as a \emph{Performer} who can, in principle, provide the most credible information to the researcher, e.g., facts about the world. The \emph{Performer's} information is expected to be more Real, Relevant and Recent (timely) compared to, for example, a requirements engineer who is an \emph{Observer}. The least credibility occurs with the requirements engineer who is an \emph{Advisor} as this participant has both the greatest variability in their experiences but also the researcher has the least certainty in the Realness, Relevance and Recentness of the \emph{Advisor's} experience and information.

As well as distinguishing roles, we recognised five characteristics of participants, as well as demographics. In different ways, these characteristics may have both a positive and a negative impact on the quality of information provided by the participants.

Finally, our distinction between three roles -- \emph{Performer}, \emph{Observer} and \emph{Advisor} -- also provides insight into some of the inherent difficulties of research strategies, e.g., a challenge with survey studies is ensuring the recruitment of \emph{Performers} in contrast to sampling \emph{Advisors}, however large the sample.

==> x_archive/X_1_introduction.tex <==
\section{Introduction}
\label{section:introduction}

\subsection{Motivation}

Software engineering research collects data from two broad sources: artefacts and people. There are at least two reasons why we collect data from software practitioners. First, many aspects of software engineering are not observable in, or through, artefacts, e.g., the context in which a software project is progressing. Because the artefacts cannot provide the data needed for the research, the researcher relies on data from people as a kind of substitute or proxy. Second, given human--centric software engineering and behavioural software engineering, researchers are interested in qualities and experiences of the people themselves, e.g., in their goals, motivation, stress, happiness, values.

There are several research methods for collecting data from people, e.g., interviews, surveys, focus groups. Fundamental to all of these methods of data collection is the need to collect data from the appropriate people. For example, an appropriate person might be someone who has direct experience of the phenomenon of interest to the researcher.

Guidelines and checklists recommend that the researcher defines a population and then draws a representative sample from, or of, that population. (It is often difficult to define a population and researchers often use a convenience sample, sometimes ‘re-engineering’ the definition of the population from the convenience sample.)

Although the advice of guidelines and checklists relates to the specification and selection of appropriate participants, we hypothesise that 1) such guidance does not provide any detailed direction on what constitutes an appropriate participant; and 2) the researcher is simply advised to select appropriate participants. Consequently, it appears that the de facto practice in software engineering research is to recruit participants based on their software engineering role, possibly also taking account of experience. For example, a researcher might survey novice requirements engineers, or interview experienced project managers, or observe a software engineering team, or select software testers for an industrial experiment. The de facto practice for case study research is necessarily different, i.e., to approach participants who are involved in some way with the case being studied, e.g., people who are members of a software project. There is however still the issue of whether the participants `selected’ in a case study are the appropriate participants given the research objectives of the case study. For example, it may not be appropriate to select a requirements engineer in a company as a participant for a case study of code reviews of software projects in that company.

This situation -- the lack of specific advice on the selection of appropriate participants -- creates considerable uncertainty in the research process, creates uncertainty about the credibility of the practitioners as participants in the respective study, and may seriously threaten the reliability and the validity of the research: if we do not have confidence that we are collecting data from credible participants (credible for that study), on what basis can we have confidence in the validity of the data those participants provide to the researcher? The uncertainties and consequent threat to reliability and validity affects all research methods that rely on participants for the collection of data, and therefore threatens the results of many already--completed research projects as well as many potential research projects in the future too.

\subsection{Scope of the paper}

To help bound our discussion, we focus this paper on the use of participants as providers of information about software phenomena that are external to the participant and that they can, in principle, observe. We include, for example, case studies, interviews and surveys of software projects. We exclude studies investigating the internal characteristics of participants, such as their motivation, or (un)happiness \cite{graziotin2017unhappiness}, or stress. Internal characteristics may affect the ability of participants to be credible observers of external behaviour.

\subsection{Contribution}

The paper makes the following contributions:
\begin{enumerate}
    \item Identify a ‘problem’ with the community’s thinking about recruiting participants, i.e., a problem with the ‘credibility’ of participants
    \item (Possible also identify a problem with the mis--framing of recruitment as about sampling, when it isn't).
    \item Shows that this problem is relevant for a wide range of types of research in SE.
    \item Proposes a framework and checklist for thinking about how to select credible participants when collecting data.
    \item Shows that the framework and checklist `fits' with three example studies, i.e., a case study, a survey study and an interview respectively. This `sense-check’ confirms that there is the need for thinking about appropriate participants.
    \item Shows that existing guidelines and checklists overlook this `problem'.
    \item Illustrates the issues with two exemplar studies and a reference study.
\end{enumerate}

\subsection{Structure of paper}

The remainder of this paper is organised as follows: \textcolor{magenta}{TBC}.

==> x_archive/X_2_old_related_work.tex <==
\section{Related work}
\label{section:related-work}

% \subsection{Introduction}
Our interest is in information that participants can provide about events \emph{external} to the participant, e.g., about the behaviour of software phenomena that the participant performs or observes. For our review of prior work, we therefore first consider, in Section \ref{subsection:participants-as-research-instruments}, the participant as a research instrument, discussing expectations of a credible participant in relation to validity, reliability, relevance, bias and accuracy. A credible participant may be understood as a key informant for empirical studies, and hence we briefly consider, in Section \ref{section:key-informants}, the \emph{key informant} as a source of information, i.e., particular participants who might provide high--quality information. Participants, particularly key informants, need to be recruited carefully and so, in Section \ref{subsection:sampling}, we turn our attention to sampling, and consider how researchers sample information about the world. Given the importance of obtaining credible information, we then consider, in Section \ref{subsection:information-flow}, the participant as a \emph{source} of information in research, and also consider the flow of that information. One essential input for our framework is the model presented by Falessi et al.~\cite{falessi2018empirical}. Thus, in Section \ref{subsection:Rmodel} we review Falessi et al.'s~\cite{falessi2018empirical} R\textsuperscript{3} model. We conclude our review with a brief summary in Section \ref{section:related-work-summary}.

\subsection{The participant as a research instrument}
\label{subsection:participants-as-research-instruments}

We can \emph{model} a participant as a kind of research instrument, or in D'Andrade's \cite{dandrade1974memory} term, as a `behaviourscope'. We can then think of the participant in terms of their reliability (how consistently they observe the world), their validity (how accurately they observe the world) and their relevance (how relevant their observations are to the research); in terms of bias; and in terms of information accuracy. We briefly consider each of these below.

\subsubsection{Validity, reliability and relevance}

Homburg et al.~\cite{homburg2012drives} used data from 127 studies across six major marketing and management journals to investigate hypotheses concerning key--informant's reliability and validity in survey studies. Homburg et al.~\cite{homburg2012drives} draw on social cognition theory to identify two concepts central to their research: (1) availability of relevant information and (2) difficulty of retrieval. The availability of relevant information and the difficulty of retrieval of information introduce random error. But they can also introduce systematic error. Where an informant lacks pertinent information or struggles to retrieve such information, these informants may provide a random best guess, thus threatening reliability; or may use some heuristic to guide their response, thus threatening validity.

\subsubsection{Bias}

Bias is already well--recognised in software engineering research. For example, Mohanani et al.~\cite{mohanani2018cognitive} report a systematic mapping study of cognitive biases in software engineering. Chattopadhyay et al.~\cite{chattopadhyay2020tale} report a two--part field study of the presence of cognitive biases in software development, drawing on the work of Mohanani et al.~\cite{mohanani2018cognitive}. Also, Mohanani et al.~\cite{mohanani2018cognitive}  cite Flesichmann et al.'s~\cite{fleischmann2014cognitive} work. We summarise biases in Table~\ref{table:cognitive-biase}.

\begin{table}[!ht]
    \small
    \caption{Cognitive bias (\cite{mohanani2018cognitive}, see also \cite{fleischmann2014cognitive})}
    \label{table:cognitive-biase}
    \centering
    \begin{tabular}{| p{0.3cm} | p{2cm} | p{10cm} | }
        % \hline
        \toprule
        \textbf{\#} & \textbf{Bias} & \textbf{Description}\\
        % \hline
        % \hline
        \midrule
        1  & Stability & Biases that lead individuals to persevere with established or familiar options despite the presence of superior information, arguments or conditions.\\
        2  & Action--oriented & Biases that lead individuals to premature decisions without considering relevant information or alternative courses of action.\\
        3 & Pattern--recognition & Biases that lead individuals to attend more to information that is familiar.\\
        4 & Perception & Biases that prejudice the processing of new information.\\
        5 & Memory & Biases that affect recall of information or experience.\\
        \bottomrule
    \end{tabular}
\end{table}

\subsubsection{Information accuracy}

Bernard et al.~\cite{bernard1984problem} are concerned with the validity and accuracy of the `naive senses' of informants.  They review previous work in three areas: recall of child care behavior; recall of health seeking behavior; and recall of communication and social interactions. They identify a number of concerns with the use of informants.  We summarise Bernard et al.'s~\cite{bernard1984problem} more relevant concerns here:

\begin{enumerate}
    % \item Informants \textit{are} inaccurate; memory \textit{does} decay exponentially with time.
    \item There appears to be systematic distortion in how informants recall just about everything.
    \item Recall may be affected by the subject of the study, by whether informants are aided in their recall in some way during, for example, an interview, by whether they keep diaries, by conditions of the interview, or by a variety of cultural factors.
    \item If informants agree with one another in information that they independently provide, then the two likely explanations are norms and actual experience.
    \begin{enumerate}
        \item When informants do not recall an actual experience, they are more likely to rely on a cultural norms for their answer.
        \item Informants who have an actual experience are more likely to resist badgering (are less likely to `back down'). A consequence is that answers that show more resistance to badgering is more likely to be accurate.
    \end{enumerate}
    \item Knowing which informants are likely to be least accurate is important. But knowing whether \emph{any} informant is sufficiently accurate is more important.
    \item Interviewing many inaccurate informants will not solve the accuracy/ validity problem, and will, as a consequence, also not produce relevant findings.
\end{enumerate}

Bernard et al.'s~\cite{bernard1984problem}'s observation about cultural norms is demonstrably present in software engineering. For example, Rainer et al.~\cite{rainer2003persuading} found that practitioners prefer local opinion over other sources of knowledge. Devanbu et al.~\cite{devanbu2016belief} conducted a large survey of Microsoft employees (n=564) finding that developers beliefs are based primarily on their personal experience and then, second, on their peers' opinions. By contrast, research papers were ranked fifth out of six. Thus, when practitioners cannot rely on their own experience they first turn to others, i.e., to the source of cultural norms. This raises a serious implication for SE research, i.e., consistency of responses across a sample of apparently independent participants may be explained by cultural norms rather than by a consistent behaviour in the phenomenona of interest.

\subsection{Key informants}
\label{section:key-informants}

Marshall~\cite{marshall1996key} defines a key informant as an expert source of information. The principal of a key informant is that the informant can provide more reliable, valid and relevant information than a sample of participants. Marshall identifies five characteristics of the ideal key informant, summarised here in Table~\ref{table:key-informants}. All five characteristics --- but particularly C1, C2 and C5 --- contribute to participant credibility. In software engineering research, an example of the use of the key informant would be the members of an expert panel, e.g.,~\cite{li2003ranking}.

\begin{table}[!ht]
    \small
    \caption{Characteristics of ideal key informant (from \cite{marshall1996key})}
    \label{table:key-informants}
    \centering
    \begin{tabular}{| l | p{12cm} | }
        \toprule
        \textbf{\#} & \textbf{Description}\\
        \midrule
        % \hline
        % \hline
        % \multicolumn{2}{|l|}{Characteristics}\\
        C1 & \textbf{Role in community}. Their formal role should expose them to the kind of information being sought by the researcher.\\
        C2 & \textbf{Knowledge}. In addition to having access to the information desired, the informant should have absorbed the information meaningfully.\\
        C3 & \textbf{Willingness}. The informant should be willing to communicate their knowledge to the interviewer and to cooperate as fully as possible.\\
        C4 & \textbf{Communicability}. They should be able to communicate their knowledge in a manner that is intelligible to the interviewer.\\
        C5 & \textbf{Impartiality}. The key informant should be objective and unbiased. Any relevant biases should be known by the interviewer, e.g., the key informant declares a bias or the interviewer can determine this from other sources.\\
        \bottomrule
    \end{tabular}
\end{table}

\subsection{Sampling}
\label{subsection:sampling}

In a recent article, Baltes and Ralph~\cite{baltes2020sampling} provide a primer on sampling. They define sampling as the process of selecting a smaller group of items to study, the \emph{sample}, from a larger group of items of interest, the \emph{population}. A \emph{sampling frame} is the available population list from which a sample can be actually drawn.

Baltes and Ralph~\cite{baltes2020sampling} identify two problems with sampling frames: first, for many software engineering phenomena there is no suitable sampling frame from which to draw a sample; second, some software engineering studies adopt poorly understood sampling strategies such as random sampling from a non--representative surrogate population. Baltes and Ralph~\cite{baltes2020sampling} also write, ``For our purposes, \emph{representativeness} is the degree to which a sample's properties (of interest) resemble those of a target population.'' (\cite{baltes2020sampling}; emphasis in original).

As noted in Section~\ref{section:introduction}, we are interested in what participants can say about software engineering phenomena they perform or observe, e.g., about software inspections or pair programming or cost estimation. In these situations, the item of interest is the phenomenon external to the participant. The participant is not the item of interest. Figuratively, the participant acts as a lens through which the researcher can observe the item of interest. A case study can illustrate this clearly, e.g., participants are interviewed for their observations of the item of interest, i.e., the case. Discussions about a sample of participants, and whether and how representative that sample may be, can therefore sometimes be misleading. We consider it helpful to also reason in terms of whether the sampled participants can provide information on a representative sample of external phenomena. 

This issue -- of the relationship of the participant to the item of interest -- does not seem to be explicitly discussed in the software engineering research literature. For case studies, the relationship appears self--evident but even there the relationship may be more complicated than assumed. For empirical studies more generally, and not just case study, there seems to be an unstated assumption, or assumptions, about the relationship between participants and items of interest (or, alternatively phrased, of units of study, or of cases). Possible assumptions might be (these are not exhaustive):
\begin{itemize}
    \item That a sufficient number and/or diversity of participants provides information on a sufficient number and/or diversity of items of interest.
    \item That a sufficiently `random' number of participants provides information on a sufficiently `random' number of items of interest.
    \item That each participant represents one item of interest.
    \item That if the study recruits `enough' participants, the study will be able to investigate `enough' items of interest.
\end{itemize}

\subsection{The flow of information in research}
\label{subsection:information-flow}

In their study of two large, independent software projects, Karlstr{\"o}m and Runeson \cite{karlstrom2006integrating} present a model of the flow of information in the research process. The \emph{source} of information for the research comes from the participants' perceptions. We present a version of Karlstr{\"o}m and Runeson's \cite{karlstrom2006integrating} model in Figure \ref{figure:generalised-karlstrom-and-runeson-figure}, simplified to make it more relevant to our article. Information about the world is collected from participant's perceptions of the world. The information is therefore transformed as it flows through the research process. This transformation may affect, amongst other qualities, the validity, reliability and relevance of the information.

\begin{figure}
    \centering
    \includegraphics[scale=0.4]{images/generalised_karlstrom_and_runeson_figure_v2.png}
    \caption{The source and flow of information in research (derived from Karlstr{\"o}m and Runeson's \cite{karlstrom2006integrating})}
    \label{figure:generalised-karlstrom-and-runeson-figure}
\end{figure}

Because Karlstr{\"o}m and Runeson \cite{karlstrom2006integrating} conduct a case study (of two cases), the participants are recruited in relation to specific, identifiable situations in the world. In Karlstr{\"o}m and Runeson's \cite{karlstrom2006integrating} study, the relationship between the participants and a set of events in the world is therefore relatively well known. A consequence is that the information that the participants are asked for is also, at least in principle, constrained. Furthermore, Karlstr{\"o}m and Runeson also interview the participants, providing the opportunity (again at least in principle) to clarify, challenge, etc. the information provided by those participants. In other words, the researchers know, or can know, something about the nature of the transformations between levels of information (at T\textsubscript{A} and T\textsubscript{B}, in Figure \ref{figure:generalised-karlstrom-and-runeson-figure}), and something about the information--selection decisions being made at levels 2 and 3.

In interview studies, the situation can be much more varied and therefore different to the Karlstr{\"o}m and Runeson \cite{karlstrom2006integrating} study. The researcher may have less influence or control on the participants recruited, e.g. using a convenience sample. Because the interview allows for interaction, the researcher may know something about the nature of transformations, may be able to influence those transformations (e.g., to challenge answers), and may be able to know and constrain something about the information-selection occurring at levels 2 and 3.

In surveys the situation is typically very different. The researcher has little, if any, influence or control on the situations in the world to which the participants refer. They also have little opportunity to influence the information provided by the participants. In other words, the researcher knows little about the nature of transformations at T\textsubscript{A} and T\textsubscript{B}, or about the information selected at level 2 and the information shared from level 2 to level 3.





==> x_archive/X_2_oldest_related_work.tex <==
\section{Related work}
\label{section:related-work}

\subsection{Introduction}
\claes{I would suggest an introduction here given the areas that we cover in related work.}

\subsection{The R\textsuperscript{3} model}
\label{subsection:Rmodel}

\claes{Summarise the model from experimentation here. I would suggest moving most of Section 4.4.1 here.}

\subsection{Sampling}
\label{subsection:sampling}

In a recent paper, Baltes and Ralph~\cite{baltes2020sampling} provide a primer on sampling. They define sampling as the process of selecting a smaller group of items to study, the \textit{sample}, from a larger group of items of interest, the \textit{population}. A \textit{sampling frame} is the available population list from which a sample can be actually drawn.

Baltes and Ralph~\cite{baltes2020sampling} identify two problems with sampling frames: first, for many software engineering phenomena there is no suitable sampling frame from which to draw a sample; second, some software engineering studies adopt poorly understood sampling strategies such as random sampling from a non--representative surrogate population. Baltes and Ralph~\cite{baltes2020sampling} also write, ``For our purposes, \textit{representativeness} is the degree to which a sample's properties (of interest) resemble those of a target population.'' (\cite{baltes2020sampling}; emphasis in original)

As noted in Section~\ref{section:introduction}, we are interested in what participants can say about software engineering phenomena they observe, e.g., about software inspections or pair programming or cost estimation. In these situations, the item of interest is the phenomenon external to the participant. The participant is not the item of interest. Figuratively, the participant acts as a lens through which the researcher can observe the item of interest. A case study can illustrate this clearly, e.g., participants are interviewed for their observations of the item of interest, the case. Discussions about a sample of participants, and whether and how representative that sample may be, can therefore be misleading. A discussion might be better directed at whether the participants can provide information on a representative sample of external phenomena. 

This issue -- of the relationship of the participant to the item of interest -- does not seem to be explicitly discussed in the software engineering research literature. For case studies, the relationship appears self--evident but even there the relationship may be more complicated than assumed. There seems to be an unstated assumption or assumptions about the relationship between participants and items of interest (or, alternatively phrased, of units of study, or of cases). Possible assumptions might be (these are not exhaustive):
\begin{itemize}
    \item That a sufficient number and/or diversity of participants provides information on a sufficient number and/or diversity of items of interest.
    \item That a sufficiently `random' number of participants provides information on a sufficiently `random' number of items of interest.
    \item That each participant represents one item of interest.
    \item That if the study recruits `enough' participants, the study will be able to investigate `enough' items of interest.
\end{itemize}

\subsection{Participants as research instruments}
\label{subsection:participants-as-research-instruments}

Our interest is in information that participants can provide about events external to the participant, e.g., about the behaviour of software phenomena that they observe. We can \textit{model} a participant as a kind of research instrument, or in D'Andrade's \cite{dandrade1974memory} term, as a `behaviourscope'. We can then think of the participant in terms of: their reliability (how consistently they observe the world) and their validity (how accurately they observe the world); in terms of bias; and in terms of information accuracy. We briefly consider each of these below.

\subsubsection{Validity, reliability and relevance}

Homburg et al.~\cite{homburg2012drives} used data from 127 studies across six major marketing and management journals to investigate hypotheses concerning key--informant's reliability and validity in survey studies. Homburg et al.~\cite{homburg2012drives} draw on social cognition theory to identify two concepts central to their research: (1) availability of relevant information and (2) difficulty of retrieval. The availability of relevant information and the difficulty of retrieval of information introduce random error. But they can also introduce systematic error. Where an informant lacks pertinent information or struggles to retrieve such information, these informants may provide a random best guess, thus threatening reliability; or may use some heuristic to guide their response, thus threatening validity.

% Relating this to the model in Figure \ref{figure:generalised-karlstrom-and-runeson-figure}:

% \begin{enumerate}
%     \item For case studies, such as the Karlstr{\"o}m and Runeson \cite{karlstrom2006integrating} reference example, we can have more confidence (in relative terms) that the participants will have relevant information as the participants are part of the cases being studied. Note that there may still be systematic error, e.g., from cultural beliefs present within the respective cases being studied.
    
%     \item In interview studies (e.g., \cite{curtis1988field}), we can have more confidence (in relative terms) that the participants will have relevant information as the participants have some relationship with the cases of interest. There may still be systematic error, though the content of that error may be different.

%     \item It surveys, it is uncertain as to whether the participants have access to relevant information.
    
% \end{enumerate}

% For reliability, Homburg et al. \cite{homburg2012drives} propose five sets of factors affecting reliability: (1) construct characteristics, (2) informant characteristics, (3) organizational characteristics, and (4) industry characteristics. Because we also investigate formal considerations, we consider method characteristics as a fifth set. For validity, Homburg et al. \cite{homburg2012drives} focus on their construct characteristics.  A summary of their results are presented in Table \ref{table:homburg-hypotheses}.

% \begin{table}[!ht]
%     \small
%     \caption{Constructs affecting reliability and validity (from  \cite{homburg2012drives})}
%     \label{table:homburg-hypotheses}
%     \centering
%     \begin{tabular}{| p{0.5cm} | p{6.6cm} | }
%         \hline
%         \textbf{\#} & \textbf{Hypothesis}\\
%         \hline
%         \hline
%         \multicolumn{2}{| l |}{Impact of constructs characteristics on \textbf{reliability}}\\
%         H1 & The reliability of key informant responses is greater for constructs pertaining to the present (vs. the past).\\
%         H2 & The reliability of key informant responses is greater for objective constructs (vs. more subjective constructs)\\
%         H3 & The reliability of key informant responses is greater for constructs pertaining to more salient events (vs. more routine events).\\
        
%         \multicolumn{2}{| l |}{Impact of informant characteristics on \textbf{reliability}}\\
%         H6 & The reliability of key informant responses is greater for informants in higher hierarchical positions (vs. lower hierarchical positions).\\
        
%         \multicolumn{2}{| l |}{Impact of method characteristics on \textbf{reliability}}\\
%         H14 & Key informant reliability estimates will be greater if triangulation is conducted using archival data (vs. survey data).\\
        
%         \multicolumn{2}{| l |}{Impact of construct characteristics on \textbf{validity}}\\
%         H16 & The validity of key informant responses is greater for constructs pertaining to the present (vs. the past).\\
%         H17 & The validity of key informant responses is greater for objective constructs (vs. more subjective constructs)\\
%         H18 & The validity of key informant responses is greater for constructs pertaining to more salient events (vs. more routine events).\\
  
%         \hline
%     \end{tabular}
% \end{table}

\subsubsection{Bias}

Mohanani et al.~\cite{mohanani2018cognitive} report a systematic mapping study of cognitive biases in software engineering. Chattopadhyay et al.~\cite{chattopadhyay2020tale} report a two--part field study of the presence of cognitive biases in software development, drawing on the work of Mohanani et al.~\cite{mohanani2018cognitive}. Mohanani et al. cite Flesichmann et al.'s~\cite{fleischmann2014cognitive} work. We summarise the biases in Table~\ref{table:cognitive-biase}.

\begin{table}[!ht]
    \small
    \caption{Cognitive bias (\cite{mohanani2018cognitive}, see also \cite{fleischmann2014cognitive})}
    \label{table:cognitive-biase}
    \centering
    \begin{tabular}{| p{0.3cm} | p{2cm} | p{10cm} | }
        % \hline
        \toprule
        \textbf{\#} & \textbf{Bias} & \textbf{Description}\\
        % \hline
        % \hline
        \midrule
        1  & Stability & Biases that lead individuals to persevere with established or familiar options despite the presence of superior information, arguments or conditions.\\
        2  & Action--oriented & Biases that lead individuals to premature decisions without considering relevant information or alternative courses of action.\\
        3 & Pattern--recognition & Biases that lead individuals to attend more to information that is familiar.\\
        4 & Perception & Biases that prejudice the processing of new information.\\
        5 & Memory & Biases that affect recall of information or experience.\\
        \bottomrule
    \end{tabular}
\end{table}

\subsubsection{Information accuracy}

Bernard et al.~\cite{bernard1984problem} are concerned with the validity and accuracy of the ``naive senses'' of informants.  They review previous work in three areas: recall of child care behavior; recall of health seeking behavior; and recall of communication and social interactions. They identify a number of concerns with the use of informants.  We summarise Bernard et al.'s~\cite{bernard1984problem} more relevant concerns here:

% As an illustrative example, we quote their summary of a study by Kornfield: ``Informants showed much higher agreement about what waiters were wearing than about what waitresses were wearing, despite the fact that none of the restaurants in question had waiters. Informants provided greater detail about the kind of music that was playing in restaurants that, in fact, did not have music than they provided for restaurants that did have music.'' (\cite{bernard1984problem}, p. 509)

\begin{enumerate}
    % \item Informants \textit{are} inaccurate; memory \textit{does} decay exponentially with time.
    \item There appears to be systematic distortion in how informants recall just about everything.
    \item Recall may be affected by the subject of the study, by whether informants are aided in their recall in some way during the interview, by whether they keep diaries, by conditions of the interview, or by a variety of cultural factors.
    \item If informants agree with one another in information that they independently provide, then the two likely explanations are norms and actual experience.
    \begin{enumerate}
        \item When informants don't recall an actual experience, they are more likely to rely on a cultural norms for their answer.
        \item Informants who have an actual experience are more likely to resist badgering (are less likely to `back down'). A consequence is that answers that show more resistance to badgering is more likely to be accurate.
    \end{enumerate}
    \item Knowing which informants are likely to be least accurate is important. But knowing whether \textit{any} informant is sufficiently accurate is more important still.
    \item Interviewing many inaccurate informants will not solve the accuracy/validity problem
\end{enumerate}

Bernard et al.'s~\cite{bernard1984problem}'s observation about cultural norms is demonstrably present in software engineering. For example, Rainer et al.~\cite{rainer2003persuading} found that practitioners prefer local opinion over other sources of knowledge. Devanbu et al.~\cite{devanbu2016belief} conducted a large survey of Microsoft employees (n=564) finding that developers beliefs are based primarily on their personal experience and then, second, on their peers' opinions. By contrast, research papers were ranked fifth out of six. Thus, when practitioners can't rely on their own experience they turn to others, i.e., to the source of cultural norms.

\subsection{Key informants}

Marshall~\cite{marshall1996key} defines a key informant as an expert source of information. The principal of a key informant is that the informant can provide more reliable and valid information than a sample of participants. Marshall identifies five characteristics of ideal key informants summarised in Table~\ref{table:key-informants}. All five characteristics (and particularly C1, C2 and C5) contribute to participant credibility. In software engineering research, an example of the use of key informants would be an expert panel, e.g.,~\cite{li2003ranking}.

\begin{table}[!ht]
    \small
    \caption{Characteristics of ideal key informants (from \cite{marshall1996key})}
    \label{table:key-informants}
    \centering
    \begin{tabular}{| l | p{12cm} | }
        \toprule
        \textbf{\#} & \textbf{Description}\\
        \midrule
        % \hline
        % \hline
        % \multicolumn{2}{|l|}{Characteristics}\\
        C1 & \textbf{Role in community}. Their formal role should expose them to the kind of information being sought by the researcher.\\
        C2 & \textbf{Knowledge}. In addition to having access to the information desired, the informant should have absorbed the information meaningfully.\\
        C3 & \textbf{Willingness}. The informant should be willing to communicate their knowledge to the interviewer and to cooperate as fully as possible.\\
        C4 & \textbf{Communicability}. They should be able to communicate their knowledge in a manner that is intelligible to the interviewer.\\
        C5 & \textbf{Impartiality}. Key informants should be objective and unbiased. Any relevant biases should be known to the interviewer\\
        \bottomrule
        % \hline
        % \multicolumn{2}{|l|}{Advantages}\\
        % A1 & Quality of data that can be obtained in a relatively short period of time. To obtain the same amount of information and insight from in-depth interviews with other members of a community can be prohibitively time-consuming and expensive\\
        % \hline
        % \multicolumn{2}{|l|}{Disadvantages}\\
        % D1 & Unlikely to represent, or even understand, the majority view of those individuals in their community.\\
        % D2 & The identification of key informants may be in error because some societies may attract people who wish to improve their status but do not have the necessary skills of a true key informant\\
        % D3 & Informants are different to informers, who are more likely to be biased and to have their own agenda.\\
        % D4 & Key informants might only divulge information that is politically acceptable and social rules could discourage the researcher from publishing potentially sensitive data which may be ascribed to a particular informant.\\
        % \hline
    \end{tabular}
\end{table}

% \subsection{Relevant knowledge}
% In this subsection we draw on Devanbu et al., Rainer et al., Hoda's paper on recruiting participants to talk about relevant knowledge.

\subsection{Summary}

We need more credible participants for our studies, i.e., informants who are more reliable and who can provide more valid information. Furthermore, the participants have to be systematically and carefully described to enable other researchers to judge the credibility of participants and the information provided by them. Such information is the foundation of empirical work that relies on practitioners, e.g., interviews, focus groups, and surveys. `Input' information from practitioners that is invalid, or information for which its validity is highly uncertain, fundamentally undermines the validity of our subsequent research findings, regardless of the reliability of the research process. Rephrasing Bernard et al.~\cite{bernard1984problem}, many studies all reporting invalid findings will not solve the problem. 

Treating the recruitment of participants as a matter of better sampling, so as to `produce' a more representative sample, is potentially mis--framing the problem. This is because participants are often not the target population. In our studies, we are often interested in what participants can tell us \textit{about} our target population, e.g., what an informant tells us about requirements engineering, or software testing, or software projects, or defects.

As a step towards addressing these concerns, we propose a framework and checklist to help researchers think about the recruitment of credible participants.

==> x_archive/X_2_related_work.tex <==
\section{Related work}
\label{section:related-work}

\austen{Add a brief explanation of how and why we structure this section the way we do.} \claes{Which we did have. I believe the reviewer also expects a motivation for the chosen sources. How do you read the comment from the reviewer?}

\subsection{The flow of information in research}
\label{subsection:information-flow}

In their study of two large, independent software projects, Karlstr{\"o}m and Runeson \cite{karlstrom2006integrating} present a model of the flow of information in the research process. The \emph{source} of information for the research comes from the participants' perceptions. We present a version of Karlstr{\"o}m and Runeson's \cite{karlstrom2006integrating} model in Figure \ref{figure:generalised-karlstrom-and-runeson-figure}, simplified to make it more relevant to our article. Information about the world is collected from participant's perceptions of the world. The information is therefore transformed as it flows through the research process. This transformation may affect, amongst other qualities, the validity, reliability and relevance of the information.

\begin{figure}
    \centering
    \includegraphics[scale=0.4]{images/generalised_karlstrom_and_runeson_figure_v2.png}
    \caption{The source and flow of information in research (derived from Karlstr{\"o}m and Runeson's \cite{karlstrom2006integrating})}
    \label{figure:generalised-karlstrom-and-runeson-figure}
\end{figure}

Because Karlstr{\"o}m and Runeson \cite{karlstrom2006integrating} conduct a case study (of two cases), the participants are recruited in relation to specific, identifiable situations in the world. In Karlstr{\"o}m and Runeson's \cite{karlstrom2006integrating} study, the relationship between the participants and a set of events in the world is therefore relatively well known. A consequence is that the information that the participants are asked for is also, at least in principle, constrained. Furthermore, Karlstr{\"o}m and Runeson also interview the participants, providing the opportunity (again at least in principle) to clarify, challenge, etc. the information provided by those participants. In other words, the researchers know, or can know, something about the nature of the transformations between levels of information (at T\textsubscript{A} and T\textsubscript{B}, in Figure \ref{figure:generalised-karlstrom-and-runeson-figure}), and something about the information--selection decisions being made at levels 2 and 3.

\austen{We might remove this paragraph to be more concise?} In interview studies, the situation can be much more varied and therefore different to the Karlstr{\"o}m and Runeson \cite{karlstrom2006integrating} study. The researcher may have less influence or control on the participants recruited, e.g. using a convenience sample. Because the interview allows for interaction, the researcher may know something about the nature of transformations, may be able to influence those transformations (e.g., to challenge answers), and may be able to know and constrain something about the information-selection occurring at levels 2 and 3.

\austen{We might remove this paragraph to be more concise?} In surveys the situation is typically very different. The researcher has little, if any, influence or control on the situations in the world to which the participants refer. They also have little opportunity to influence the information provided by the participants. In other words, the researcher knows little about the nature of transformations at T\textsubscript{A} and T\textsubscript{B}, or about the information selected at level 2 and the information shared from level 2 to level 3.

\subsection{Sampling}
\label{subsection:sampling}

In a recent article, Baltes and Ralph~\cite{baltes2020sampling} provide a primer on sampling. They define sampling as the process of selecting a smaller group of items to study, the \emph{sample}, from a larger group of items of interest, the \emph{population}. A \emph{sampling frame} is the available population list from which a sample can be actually drawn.

Baltes and Ralph~\cite{baltes2020sampling} identify two problems with sampling frames: first, for many software engineering phenomena there is no suitable sampling frame from which to draw a sample; second, some software engineering studies adopt poorly understood sampling strategies such as random sampling from a non--representative surrogate population. Baltes and Ralph~\cite{baltes2020sampling} also write, ``For our purposes, \emph{representativeness} is the degree to which a sample's properties (of interest) resemble those of a target population.'' (\cite{baltes2020sampling}; emphasis in original).

As noted in Section~\ref{section:introduction}, we are interested in what participants can say about software engineering phenomena they perform or observe, e.g., about software inspections or pair programming or cost estimation. In these situations, the item of interest is the phenomenon external to the participant. The participant is not the item of interest. Figuratively, the participant acts as a lens through which the researcher can observe the item of interest. A case study can illustrate this clearly, e.g., participants are interviewed for their observations of the item of interest, i.e., the case. Discussions about a sample of participants, and whether and how representative that sample may be, can therefore sometimes be misleading. We consider it helpful to also reason in terms of whether the sampled participants can provide information on a representative sample of external phenomena. 

This issue -- of the relationship of the participant to the item of interest -- does not seem to be explicitly discussed in the software engineering research literature. For case studies, the relationship appears self--evident but even there the relationship may be more complicated than assumed. For empirical studies more generally, and not just case study, there seems to be an unstated assumption, or assumptions, about the relationship between participants and items of interest (or, alternatively phrased, of units of study, or of cases). Possible assumptions might be (these are not exhaustive):
\begin{itemize}
    \item That a sufficient number and/or diversity of participants provides information on a sufficient number and/or diversity of items of interest.
    \item That a sufficiently `random' number of participants provides information on a sufficiently `random' number of items of interest.
    \item That each participant represents one item of interest.
    \item That if the study recruits `enough' participants, the study will be able to investigate `enough' items of interest.
\end{itemize}

\subsection{Key informants}
\label{section:key-informants}

Marshall~\cite{marshall1996key} defines a key informant as an expert source of information. The principal of a key informant is that the informant can provide more reliable, valid and relevant information than a sample of participants. Marshall identifies five characteristics of the ideal key informant, summarised here in Table~\ref{table:key-informants}. All five characteristics --- but particularly C1, C2 and C5 --- contribute to participant credibility. In software engineering research, an example of the use of the key informant would be the members of an expert panel, e.g.,~\cite{li2003ranking}.

\begin{table}[!ht]
    \small
    \caption{Characteristics of ideal key informant (from \cite{marshall1996key})}
    \label{table:key-informants}
    \centering
    \begin{tabular}{| l | p{12cm} | }
        \toprule
        \textbf{\#} & \textbf{Description}\\
        \midrule
        % \hline
        % \hline
        % \multicolumn{2}{|l|}{Characteristics}\\
        C1 & \textbf{Role in community}. Their formal role should expose them to the kind of information being sought by the researcher.\\
        C2 & \textbf{Knowledge}. In addition to having access to the information desired, the informant should have absorbed the information meaningfully.\\
        C3 & \textbf{Willingness}. The informant should be willing to communicate their knowledge to the interviewer and to cooperate as fully as possible.\\
        C4 & \textbf{Communicability}. They should be able to communicate their knowledge in a manner that is intelligible to the interviewer.\\
        C5 & \textbf{Impartiality}. The key informant should be objective and unbiased. Any relevant biases should be known by the interviewer, e.g., the key informant declares a bias or the interviewer can determine this from other sources.\\
        \bottomrule
    \end{tabular}
\end{table}

\subsection{The participant as a research instrument}
\label{subsection:participants-as-research-instruments}

We can \emph{model} a participant as a kind of research instrument, or in D'Andrade's \cite{dandrade1974memory} term, as a `behaviourscope'. We can then think of the participant in terms of their reliability (how consistently they observe the world), their validity (how accurately they observe the world) and their relevance (how relevant their observations are to the research); in terms of bias; and in terms of information accuracy. We briefly consider each of these below.

\subsubsection{Validity, reliability and relevance}

Homburg et al.~\cite{homburg2012drives} used data from 127 studies across six major marketing and management journals to investigate hypotheses concerning key--informant's reliability and validity in survey studies. Homburg et al.~\cite{homburg2012drives} draw on social cognition theory to identify two concepts central to their research: (1) availability of relevant information and (2) difficulty of retrieval. The availability of relevant information and the difficulty of retrieval of information introduce random error. But they can also introduce systematic error. Where an informant lacks pertinent information or struggles to retrieve such information, these informants may provide a random best guess, thus threatening reliability; or may use some heuristic to guide their response, thus threatening validity.

\subsubsection{Bias}

Bias is already well--recognised in software engineering research. For example, Mohanani et al.~\cite{mohanani2018cognitive} report a systematic mapping study of cognitive biases in software engineering. Chattopadhyay et al.~\cite{chattopadhyay2020tale} report a two--part field study of the presence of cognitive biases in software development, drawing on the work of Mohanani et al.~\cite{mohanani2018cognitive}. Also, Mohanani et al.~\cite{mohanani2018cognitive}  cite Flesichmann et al.'s~\cite{fleischmann2014cognitive} work. We summarise biases in Table~\ref{table:cognitive-biase}.

\begin{table}[!ht]
    \small
    \caption{Cognitive bias (\cite{mohanani2018cognitive}, see also \cite{fleischmann2014cognitive})}
    \label{table:cognitive-biase}
    \centering
    \begin{tabular}{| p{0.3cm} | p{2cm} | p{10cm} | }
        % \hline
        \toprule
        \textbf{\#} & \textbf{Bias} & \textbf{Description}\\
        % \hline
        % \hline
        \midrule
        1  & Stability & Biases that lead individuals to persevere with established or familiar options despite the presence of superior information, arguments or conditions.\\
        2  & Action--oriented & Biases that lead individuals to premature decisions without considering relevant information or alternative courses of action.\\
        3 & Pattern--recognition & Biases that lead individuals to attend more to information that is familiar.\\
        4 & Perception & Biases that prejudice the processing of new information.\\
        5 & Memory & Biases that affect recall of information or experience.\\
        \bottomrule
    \end{tabular}
\end{table}

\subsubsection{Information accuracy}
\label{section:accuracy}

Bernard et al.~\cite{bernard1984problem} are concerned with the validity and accuracy of the `naive senses' of informants.  They review previous work in three areas: recall of child care behavior; recall of health seeking behavior; and recall of communication and social interactions. They identify a number of concerns with the use of informants.  We summarise Bernard et al.'s~\cite{bernard1984problem} more relevant concerns here:

\begin{enumerate}
    % \item Informants \textit{are} inaccurate; memory \textit{does} decay exponentially with time.
    \item There appears to be systematic distortion in how informants recall just about everything.
    \item Recall may be affected by the subject of the study, by whether informants are aided in their recall in some way during, for example, an interview, by whether they keep diaries, by conditions of the interview, or by a variety of cultural factors.
    \item If informants agree with one another in information that they independently provide, then the two likely explanations are norms and actual experience.
    \begin{enumerate}
        \item When informants do not recall an actual experience, they are more likely to rely on a cultural norms for their answer.
        \item Informants who have an actual experience are more likely to resist badgering (are less likely to `back down'). A consequence is that answers that show more resistance to badgering is more likely to be accurate.
    \end{enumerate}
    \item Knowing which informants are likely to be least accurate is important. But knowing whether \emph{any} informant is sufficiently accurate is more important.
    \item Interviewing many inaccurate informants will not solve the accuracy/ validity problem, and will, as a consequence, also not produce relevant findings.
\end{enumerate}

Bernard et al.'s~\cite{bernard1984problem}'s observation about cultural norms is demonstrably present in software engineering. For example, Rainer et al.~\cite{rainer2003persuading} found that practitioners prefer local opinion over other sources of knowledge. Devanbu et al.~\cite{devanbu2016belief} conducted a large survey of Microsoft employees (n=564) finding that developers beliefs are based primarily on their personal experience and then, second, on their peers' opinions. By contrast, research papers were ranked fifth out of six. Thus, when practitioners cannot rely on their own experience they first turn to others, i.e., to the source of cultural norms. This raises a serious implication for SE research, i.e., consistency of responses across a sample of apparently independent participants may be explained by cultural norms rather than by a consistent behaviour in the phenomenon of interest.

\subsection{The R\textsuperscript{3} model}
\label{subsection:Rmodel}

Falessi et al.~\cite{falessi2018empirical} propose the R\textsuperscript{3} model comprising three elements of a subject's experience: Real, Relevant and Recent. The R\textsuperscript{3} model was formulated for experiments. We summarise the R\textsuperscript{3} model here and then reformulate it in Section \ref{section:framework} to align with our proposed framework.
% , i.e., the three characteristics are relevant for identifying practitioners -- possibly key informants -- who are more likely to be good sources of information for research.

The three elements of the R\textsuperscript{3} model are: 
\begin{itemize}
    \item That the subject has \emph{real experience} of software engineering situations. It is not possible to provide a formal definition for `real experience'. Broadly speaking, `real experience' refers to experience of situations of real--world software practice that are, in general, of interest to the research.
    \item That the subject has \emph{relevant experience}. Relevance here refers to the `fit' between the situation and the research model. The characteristic of relevance becomes more significant for a type of informant we discuss later in this article, i.e., the \emph{advisor}.
    \item That the subject has \emph{recent experience}, or more precisely \emph{timely experience}, e.g., typically that the situation has been experienced recently by the subject, relative to the focus of the research.
\end{itemize}

All three of the above elements need to be tailored, by the researcher, to the specific needs of the respective research. The researcher will also need to assess each subject against each of the (possibly tailored) elements.

\subsection{Summary}
\label{section:related-work-summary}
\austen{This needs reworking}

We need more, and more--credible, participants for our empirical studies, i.e., more informants who are more reliable and who can provide more valid and relevant information in relation to the research being conducted. Furthermore, the participants have to be systematically and carefully described to enable other researchers to judge the credibility of participants and the information provided by them. Such information is the foundation of empirical work that relies on practitioners, e.g., interviews, focus groups, and surveys. `Input' information from practitioners that is invalid, or information for which its validity is highly uncertain, fundamentally undermines the validity of our subsequent research findings, regardless of the reliability of the research process. Rephrasing Bernard et al.~\cite{bernard1984problem}, many studies all reporting invalid findings will not solve the credibility problem. 

Treating the recruitment of participants as a matter of better sampling, so as to `produce' a more representative sample, is potentially mis--framing the problem. This is because participants themselves are often not the item of \emph{research} interest. In our studies, we are often interested in what participants can tell us \emph{about} the items of research interest, e.g., what an informant tells us about requirements engineering, or software testing, or software projects, or defects. The distinction between the participant and the item of interest is also important because of the effects of cultural norms, e.g., a participant may provide a culturally--normative response because the participant has not reliably observed or performed the item of interest and cannot provide valid information on that item of interest.

As a step towards addressing these concerns, we propose a framework to help researchers think about the recruitment of credible participants. We also provide a preliminary checklist in Appendix A.

==> x_archive/X_3_illustrative_examples.tex <==
\section{Illustrative examples}
\label{section:X_3}

We discuss two papers as illustrative examples of the issues we explore. These two papers are selected because of the  level of detailed explanation reported in the respective papers. The first paper, by Karlstr{\"o}m and Runeson \cite{karlstrom2006integrating}, presents a case study. The second paper, by Schermann et al. \cite{SCHERMANN201841}, presents two interview studies and a survey study. 

\subsection{Case study example}
\label{subsection:reference-example}

Karlstr{\"o}m and Runeson \cite{karlstrom2006integrating} present a study of two large, independent software projects that use eXtreme Programming within a stage--gate project management model. Our interest in their study is in the way that they reason about the research process.  We use their study as a reference example in our paper.

Karlstr{\"o}m and Runeson present a model of the information used in the study and of the transformation of that information. They discuss threats to the validity of the research that arise as the information is transformed. They also discuss strategies for dealing with those threats. For convenience of comparison, Karlstr{\"o}m and Runeson’s model of information--transformation is reproduced here in Figure \ref{figure:karlstrom-and-runeson-figure}. Our paper focuses on the lowest three levels of their model but also generalises those three levels beyond case study research. We also re-label the model. We present our more generalised version in Figure \ref{figure:generalised-karlstrom-and-runeson-figure}.

\begin{figure}
    \centering
    \includegraphics[scale=0.8]{images/karlstrom_and_runeson_figure.png}
    \caption{Karlstr{\"o}m and Runeson \cite{karlstrom2006integrating} levels and transformation of information in their research process}
    \label{figure:karlstrom-and-runeson-figure}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale=0.4]{images/generalised_karlstrom_and_runeson_figure_v1.png}
    \caption{Generalised version of the lower three levels of Karlstr{\"o}m and Runeson's \cite{karlstrom2006integrating} research process. \textcolor{magenta}{Rework as a table?}}
    \label{figure:generalised-karlstrom-and-runeson-figure}
\end{figure}

Many of the threats and strategies discussed by Karlstr{\"o}m and Runeson relate to higher levels of their model, and therefore are not relevant for our discussion. Also, the threats and strategies that Karlstr{\"o}m and Runeson do identify for the lower levels are different to those we identify. For these reasons, we do not reproduce their tables of threats and strategies here.

Karlstr{\"o}m and Runeson study two cases, EMW and ABB. Participants are therefore recruited in relation to specific, identifiable situations in the world. A consequence is that the information that the participants are asked for is also, at least in principle, constrained. Furthermore, Karlstr{\"o}m and Runeson also interview the participants, providing the opportunity (again at least in principle) to clarify, challenge etc. the information provided by those participants. In order words, the researchers know (or can know) something about the nature of transformations TA and of TB, and something about the information-selection decisions being made at levels 1, 2 and 3.

In interview studies, the situation can be much more varied and therefore different to the Karlstr{\"o}m and Runeson study. The researcher may have less influence or control on the participants recruited, e.g. using a convenience sample. Because the interview allows for interaction, the researcher may know something about the nature of transformations TA and of TB, (and may be able to influence those transformations) and may be able to know and constrain something and the information-selection occurring at levels 1, 2 and 3.

In surveys the situation is typically very different. The researchers have little, if any, influence or control on the situations in the world to which the participants refer. They also have little opportunity to influence the information provided by the participants. In order words, the researchers knows little about the nature of transformations TA and of TB, or about the information-selection at level 1 and 2.

By contrast, observational studies allow the researcher much greater control. Indeed, the participants may not be treated as research instruments in the way they are used as research instruments for case study, survey and interview.

\subsection{Interviews and survey}

Schermann et al. \cite{SCHERMANN201841} report a multi--method empirical study on continuous experimentation in software development companies. Their multi--method study comprises two interview studies and a survey study. The paper is valuable as an illustrative example for several reasons: they explain the overall research methodology; they explain the participant recruitment and sample for each study; they discuss threats to validity for each study; they provide a detailed appendix with further information on the design and conduct of the studies; and, finally, they complement the published paper with an online supplement. For simplicity we focus here on their first interview study and their survey study (our discussion of their first interview study we essentially be repeated for their second interview study). These two studies are summarised in Table \ref{table:multi-method-illustrative-example}. 

The research questions for their multi--method study were:
\begin{itemize}
    \item RQ1 : What principles and practices enable and hinder organizations to leverage continuous experimentation?
    \item RQ2 : What are the different flavors of continuous experimentation and how do they differ?
\end{itemize}

\subsubsection{First interview study}

In their discussion of the threats to the first interview study, Schermann et al. write, ``\dots a potential threat to our empirical findings is that our results are not generalizable beyond the subjects involved\dots'' (\cite{SCHERMANN201841}, p. 46). Elsewhere, also in relation to the first interview study, the paper says, ``Snowball sampling helped us to increase our sample size'' (\cite{SCHERMANN201841}, p. 46). Given the two research questions, that the multi--method study is focused on experimentation in software development, and the different types of case (i.e., individual, process, team, company; see Table \ref{table:multi-method-illustrative-example}), it is not clear why generalisation would be on the basis of \textit{participants}.

To be fair, Schermann et al. \cite{SCHERMANN201841} recognise there is a threat to generalisability. Their mitigation of that threat is through the mixed--method approach: ``We mitigate this effect by employing a mixed--method study validating our interview findings in a more general context using a quantitative survey in the following step.'' (\cite{SCHERMANN201841}, p. 46).

We suggest that the 20 participants might better be understood as a kind of \textit{sampling frame} (cf. the discussion of sampling in Section \ref{subsection:sampling}) through which a sample of real--world phenomena are indirectly studied. The difficulty is that it remains unclear what `units' of phenomena are being studied `through' these participants. Or in other words, what is the case from which one seeks to generalise (either analytically or statistically)?

\begin{table}[!ht]
    \small
    \caption{Summary of Schermann et al.'s multi--method study \cite{SCHERMANN201841}}
    \label{table:multi-method-illustrative-example}
    \centering
    \begin{tabular}{| p{1.5cm} | p{5.7cm} | }
        \hline
        \textbf{Dimension} & \textbf{Description}\\
        \hline
        \hline
        \multicolumn{2}{|l|}{First interview study}\\
        \hline
        Recruitment process & From industry partners, personal networks and snowballing.\\
        \hline
        Sample & ``to recruit interview participants that are approximately evenly distributed between organizations of varying sizes, divergent domains, and backgrounds (years of experience and age of participants)'' (p. 46)\\
        \cline{2-2}
        & 20 participants: Software Engineer, DevOps Engineer, Solution Architect, Public Cloud Architect, Program Manager, Project Lead, Director of Engineering\\
        \cline{2-2}
        & 3 company types: Startup, SME, Corporate\\
        \cline{2-2}
        & 4 applications types: Web, Enterprise, Desltop, Embedded\\
        \cline{2-2}
        & \textcolor{magenta}{X application domains: \dots}\\
        \cline{2-2}
        & 6 countries: Austria, Germany, Switzerland, Ireland, Ukraine, \& the US.\\
        \hline
        Case/s & 4 types: Individual, process, team, company\\
        \hline
        Data \mbox{collection} & Topics followed the natural flow of the interview.\\
        \cline{2-2}
        & Not all questions were asked of all participants.\\
        \hline
        Threats & ``\dots we rely on self--reported (as opposed to observed) behavior and practices (self--reporting bias).'' (p. 46)\\
 
        \hline     
        \hline
        \multicolumn{2}{|l|}{Survey study}\\
        \hline
        Recruitment process & distributed the survey within  personal networks, social media, via two DevOps related newsletters, and via a German-speaking IT news portal.\\
        \hline
        Sample & 187 respondents\\
        \cline{2-2}
        & Experience: 8yrs average (4yrs SD)\\
        \hline
        Case/s & Similar to the interviews, some questions focused on the development and deployment process on the team or company level\\
        \cline{2-2}
        & 3 company types: Startup, SME, Corporate\\
        \cline{2-2}
        & 6 application types: Embedded, Mobile, Desktop, Enterprise, Web, Other\\
        \hline
        Threats & it is likely that the survey has attracted a respondent demography with substantial interest and familiarity with continuous deployment and experimentation practices (self--selection bias).\\
        \cline{2-2}
        & participants may have provided idealized data about their companies’ states on CD and experimentation (self--reporting bias).\\
        
        % \hline
        % \hline
        % \multicolumn{2}{|l|}{Second study}\\
        % Participant recruitment & \\
        % Sample & 11 participants: Software Engineer, DevOps Engineer, Head of Department, Team Lead, Head Release Engineering, Director of Engineering\\
        % & 3 company types: Startup, SME, Corporate\\
        % & 1 applications type: Web\\
        % & X application domains: \dots\\
        % & 4 countries: Germany, Ukraine, UK, \& the US.\\
        % Case/s & \\ 
        
        \hline
    \end{tabular}
\end{table}

\subsubsection{Survey study}

In the appendix to their paper, Schermann et al. \cite{SCHERMANN201841} write, ``\dots in surveys subjects are sampled from a population to which results are intended to be generalized.'' (\cite{SCHERMANN201841}, p. 55). As with the first interview study, it is not clear whether participants are the appropriate \textit{population} from which to sample items (i.e., participants). 

\subsection{Summary}

\textcolor{magenta}{To be written.}

==> x_archive/X_4_original_framework.tex <==
\section{Framework [Original]}
\label{section:framework-and-checklist}

In this section we present and discuss the framework for recruiting credible practitioners.

The framework comprises four main components: situations of interest, research models, informants and their characteristics, and research strategies to collect information. In terms of research strategies, we focus on case study, interview study and survey study. Strictly speaking, the experiment provides for the most control in an empirical study and therefore the most control of the relationship between participant and item of interest. We focus here on studies that occur outside of the laboratory environment; or in other words on different types of field study. Also, our focus here is on controlling the relationship between participant and item of interest, not on other aspects of the study. 

We complement the framework with a checklist, presented in Appendix A. The checklist provides a set of questions, derived from the framework, to `ask' of actual empirical studies, whether these studies are in preparation, in conduct, or completed. 

\subsection{Situations as items of interest}

The concept \emph{item of interest} is abstract so in this section we explain the more specific types of items that concern us in this paper.

A software practitioner is typically located somewhere within a software engineering situation and experiences that situation. For simplicity, we use four constructs to describe the situation: the \emph{actor}, the \emph{technology}, the \emph{activity} and the \emph{software artefact}. These constructs are well--accepted in software engineering research~\cite{sjoberg2008building}. These constructs exist within a \emph{context} \cite{petersen2009context, dybaa2012works, clarke2012situational} which, by its nature, is difficult to define. We consider context later in this section. For convenience, we collectively refer to the four constructs using the acronyms ATAS, or sometimes with the acronym ATASC when we want to also include context. 

Sometimes a software practitioner who is located outside of the situation can provide important information about the situation. These `outside practitioners' may have experience of software practice that has some relevance to the situation of interest and to the research. For example, while the total ATAS configuration for the outside practitioner may be different, there may be some part of the configuration that is directly relevant, such as the relationship between the \emph{technology} and \emph{activity} being considered in the research. The information provided by these outside practitioners may therefore be relevant to the research through inference, however formal or informal the inference. For these `outside practitioners', it is not clear whether they have experienced any of the items of interest, i.e., whether they legitimately are part of the sampling frame.

\subsection{Relationship of participants and items of interest}

As noted in Section~\ref{section:related-work}, the relationship of the recruited participant to the item of interest in an empirical study does not seem to be explicitly discussed in the software engineering research literature. 

\begin{figure}
    \centering
    \includegraphics[scale=0.4]{images/participants-as-sampling-frame-v2.png}
    \caption{Participants as a sampling frame. Each participant has access to one or more items of interest from the population, and the aggregate of participants provides a sampling frame.}
    \label{figure:participants-as-a-sampling-frame}
\end{figure}

We suggest that it may be more effective to treat participants as a kind of sampling frame through which items from the population of real--world phenomena are sampled and then indirectly studied. Our `logic' of participants as a sampling frame is illustrated in Figure \ref{figure:participants-as-a-sampling-frame} and discussed briefly below in relation to three common types of empirical study.

\subsubsection{Case studies}

A case study (as defined by \cite{wohlin2021case} and \cite{yin1994case}, and exemplified by \cite{runeson2009guidelines}) is something of a special case. In a case study, multiple participants are typically interviewed about one item of interest. Where there are multiple case studies, multiple participants may be interviewed for each case. It is the case study that typically provides more control on the relationship between participant and item of interest.

Sometimes a study is presented as a case study when, for example, it is, more accurately, an interview study~\cite{wohlin2021case}. These studies investigate specific cases (items of interest), clearly map interviewees to cases and are therefore studies of cases. But such studies are not case studies, e.g., because they do not satisfy the other full set of criteria for a case study \cite{wohlin2021case}, or because they might only interview one participant about each case.

\subsubsection{Interview studies}

In a typical interview study, each interviewee provides indirect access to a (usually unknown) number of items of interest. Sometimes the interview study is designed to control the relationship between respondent and item of interest, e.g., the respondent is asked to respond in relation to only one item of interest that they have experienced.

In an interview study, the researcher may knowingly interview more than one interviewee about a common item of interest, e.g., two people are interviewed about their experience of one software project, or both programmers are interviewed about their shared pair programming sessions. Also, because the interview provides for interaction, the researcher has greater control (or at greater least influence) than, for example, with surveys, to ensure the interviewee maintains the required relationship with the item/s of interest.

\subsubsection{Survey studies}

In a typical survey study, and like the typical interview study, each respondent to the survey provides indirect access to a (usually unknown) number of items of interest. For example, each respondent may have experience of one or more software projects, or one or more software inspections. Sometimes, a survey study will be designed to try to control the relationship between respondent and item of interest. For example, the respondent may be asked to respond only on the basis of the most recently experienced item from the population, such as the most recently completed software project. 

\subsubsection{Summary}

Overall, the relationship between participant and item of interest varies, or at least can vary, between the different kinds of research strategy. For example, there can be a many--to--many, one--to--many or many--to--one relationship.

\subsection{Research model}

For an empirical study, a researcher usually has a research question or similar (e.g., hypothesis or proposition) together with some conceptual or theoretical foundation, however explicitly or implicitly defined, for that research question. For simplicity, we refer to the research question and its related constructs as the \emph{research model}.

The research model relates, explicitly or implicitly, to a situation or situations. Broadly speaking, the model may offer a description, explanation, prediction or some control for one or more situations or parts of those situations~\cite{sjoberg2008building} and~\cite{stol2015theory}. As one example, consider a research model comprising a set of critical success factors for software projects. In this example, the critical success factors provide some kind of prediction of the final outcome of one or more software projects. A specific project may be a situation of interest to a specific practitioner, and either specific projects or an aggregate of projects may be items of interest to the researcher.

Like all models, the research model will have properties such as its scope and resolution. We do not need to consider the full range of properties of the research model here however we do need to recognise three properties: abstraction, `distance’ and `proximity’. Depending on the level of abstraction, two situations may be more similar or less similar and taken to extremes all situations may be considered identical (e.g., they are all generic software engineering phenomena) or alternatively each situation may be considered entirely unique (e.g., each is an individual phenomenon in its own right).

The property of abstraction leads to the properties of `distance’ (e.g.,~\cite{bjarnason2016theory}) and of `proximity'. Most of these `distances' and `proximities' are not physical. Again, it is not possible to anticipate all possible types of distance or proximity, or consider how distance and proximity should be measured; and, again, it is not necessary for the current paper to consider all these types and measures. There are, however, three distance/proximity relationships of significance for this paper:
\begin{itemize}
    \item The distance between situations and therefore the proximity of situations;
    \item The distance between each situation and the research model;
    \item The distances between informants and therefore the proximity of informants;
\end{itemize}

The third relationship -- the proximity of informants -- is similar to demographics. We discuss demographics later in this section.

It is the responsibility of the respective researcher to handle such properties in the research models of their research.

A practitioner may experience several situations; indeed experience of an increasing number of situations is part of what it means to be a more experienced practitioner. There is then the challenge to the researcher (and perhaps to the practitioner) to decide how close (cf. proximity) these situations are to the research model. Similarly, multiple practitioners may each experience their own respective situation (or situations) and, again, there is the challenge to the researcher (and perhaps to the practitioner) to decide how close each situation is to the research model.

Relating this back to populations, samples and sampling frames, the properties of the research model (e.g., scope, resolution, and abstraction) should influence the specification of the sampling frame. For example, a study that investigates requirements engineering for web applications would use those two characteristics to help specify the kinds of items of interest in the sampling frame. A candidate participant may have experience of non--web applications. \emph{Ideally}, these experiences should be filtered out, either through the recruitment process (the candidate is not included in the study) or then through the sampling frame (some of the experiences of the recruited participant are not used in the study).

\subsection{Informants and their information--providing characteristics}

Given the preceding discussion, we consider several characteristics for recruiting practitioners as informants.

\subsubsection{Roles}
\label{subsubsection:roles}

In Section \ref{section:related-work}, we discussed Falessi et al.'s~\cite{falessi2018empirical} R\textsuperscript{3} model comprising three characteristics, i.e., Real, Relevant, and Recent. Accepting that a practitioner satisfies these three characteristics, there is a further set of characteristics that concern the \emph{role} of the informant. We define three roles here (specific studies may need to define additional roles for the respective study, or an alternative set of roles):
\begin{itemize}
    \item The practitioner who is an \emph{actor} within the situation, i.e., the practitioner is the actor (or one of the actors) for the ATAS configuration.
    \item The practitioner who is an \emph{observer}, but not an actor, and is located elsewhere within the situation. It is not possible, or necessary, to be precise in this paper about where the observer is located in that situation.
    \item The practitioner who is an \emph{advisor} with sufficient experience of other situations for the advisor's experience to have value to the research. The more experienced, and the more widely experienced, a software practitioner becomes the more likely they will have \emph{some} real experience of relevance to the research (though, as we recognised, some of that experience may not be recent). The role of \emph{advisor} relates to our earlier discussion on `outside practitioners'.
\end{itemize}

In reality, some of the practitioner's experience may allow that practitioner to be classified as an \emph{actor}, whilst some other of the same practitioner's experience may allow that practitioner to be classified as an \emph{observer}, and yet some other of the same practitioner's experience may allow that practitioner to be classified as an \emph{advisor}; and indeed some of the practitioner's experience may not allow classification according to the three roles (e.g., because that experience is not relevant). We acknowledge this complication: it is a complication inherent within software development.

Our suggestion is that the researcher evaluates an informant against these three roles in the order that we have presented them, i.e., first determine whether the informant could be treated as \emph{actor}. According to our framework, an informant who could not satisfy any of the three roles would in principle be rejected as an informant. In practice, the researcher may introduce an additional role or roles of informant, where it is appropriate to do so for their research.

\subsubsection{Additional characteristics}
\label{sec:characteristics}

There are five further characteristics of the informant to consider. These characteristics are partly derived from Marshall's~\cite{marshall1996key} five characteristics of a key informant, summarised in Table \ref{table:key-informants} in Section \ref{section:key-informants}. First, the informant must have the willingness or, alternatively phrased, the motivation to share information. Second, and in general, the greater the quantity of situations experienced by the informant, the more experienced is the informant for the research. Third, the more the informant is able to \emph{carefully} observe events and, through that careful observation, to help prevent or reduce bias in their observation, the more valuable is the informant for the research. Fourth, the more the informant is able to subsequently \emph{reflect} on those observations as they develop their experience and, through that reflection, to help prevent or reduce biases in the information they share with the researchers, the more valuable is the informant for the research. Fifth, and finally, the more the informant can distinguish between the situations and so provide only the more valid and relevant information to the researcher, the more valuable is the informant for the research. For the last characteristic, it may be more valuable to the researcher for the informant to \emph{restrict} the information they share to a specific situation, or situations, to ensure the information is more valid and more relevant (cf. the role of the  sampling frame). And it is, of course, a responsibility of the researcher to support the informant in that recruitment process.

These five characteristics -- of willingness, of quantity of experience, of observational ability, of reflective ability, and of situation selection -- are all simplifications, and are all very challenging to measure. Again, the principle here is that we seek informants who are able to provide more valid and more relevant information to the research. 

\subsubsection{Demographics}

Empirical studies of software engineering often report the demographics of the informants. For example, in one of their survey studies of professional software engineers at Microsoft, Begel and Zimmerman~\cite{begel2014analyze} found statistically significant differences in responses to 29 questions, based on the demographics of the respondents. And taking one pervasive demographic -- gender -- as a another example, Carver and Serebrenik~\cite{carver2019} summarise several papers published in the 2019 edition of the International Conference on Software Engineering (ICSE) that discuss gender and software engineering.

These examples highlight the importance of considering demographics when collecting information from informants about their experience of software practice, i.e., informants with differing demographics may have differing experiences and may therefore provide different information. Also, it may be that the three roles we have identified have different demographic profiles, e.g., different proportions of gender or age.

As noted earlier, demographics may be treated as one or more dimensions when considering the distance and proximity of informants to each other. Because of the inherent nature of demographics, and because of the pervasiveness of collecting demographic information in software engineering research, we explicitly recognise demographics in our framework, rather than only implying it in the existing characteristics.

\subsubsection{Additional considerations}
\label{section:additional-considerations}

When applying the framework some additional considerations will need to be addressed. As one example, using some kind of key informant in research potentially reduces the number of participants and therefore increases the likelihood that the informant/s might be identifiable, e.g., when conducting an interview study in a company. This raises ethical issues. We do not consider these issues in this paper, however Strandberg~\cite{Strandberg2019}, for example, discusses ethical issues affecting interviews in software engineering. As a second example, \emph{finding} key informants may be challenging, particularly as the researcher becomes more selective on the characteristics of the participant. But, as we noted from Bernard et al.'s~\cite{bernard1984problem} work in Section~\ref{section:related-work}, collecting information from many inaccurate participants will not solve the accuracy/validity problem, and will, as a consequence, also not produce relevant findings.

\subsubsection{Summary}

To summarise, we propose a framework with the following, twelve characteristics:
\begin{itemize}
    \item The three characteristics of real, relevant and timely experience.
    \item The three roles of informant, i,.e., actor, observer and advisor.
    \item The five characteristics of willingness, quantity of experience, observational ability, reflective ability, and situation selection.
    \item A collection of demographics.
\end{itemize}

We recognise that it may not be straightforward to classify practitioners according to these characteristics, and also that there may be other legitimate characteristics to consider. The difficulty of classifying practitioners is a natural consequence of the complexity of software engineering research.

These characteristics are intended to help the researcher decide whether a candidate participant will contribute to the formation of a coherent sampling frame. 

\subsection{Context}

Earlier in this section we chose four constructs to describe the situation, the \emph{actor}, the \emph{technology}, the \emph{activity} and the \emph{software artefact}. We also recognised \emph{context}. Broadly speaking, \emph{context} refers to other constructs that may be relevant to the research but are not considered by the research. Each empirical study may have important constructs for describing the situation that we do not consider in our framework.

Also, constructs may be related in different ways depending on the interests of the practitioner and of the researcher. It is not possible, or necessary, for our paper to anticipate all the constructs that may be important, or all the ways in which practitioners or researchers might relate these constructs to each other. But we do need to recognise the presence and influence of context in research.

\subsection{Types of information}

The researcher seeks information, from informants and about situations, that the researcher can use with their research model. Broadly speaking, there are two types of information the researcher may collect from informants:

\begin{enumerate}
    \item Empirical information, e.g., descriptive information about specific situations (items of interest).
    \item Conceptual information, e.g., opinions, hypotheses, theories formed from one situation or more than one situation.
\end{enumerate}

In principle (and this may be difficult in practice), the three informant roles -- \emph{actor}, \emph{observer} and \emph{advisor} -- can provide different kinds of information:
\begin{enumerate}
    \item The actor and the observer can each, from different perspectives, provide empirical information of specific situations.
    \item The actor and the observer can each, again from different perspectives, provide conceptual information. Such conceptual information, e.g., opinions, can be drawn from either specific situations, or from some aggregate of situations.
    \item The advisor can provide conceptual information, this information can be drawn from either specific but distant situations, or from some aggregate of these distant situations.
\end{enumerate}

Similarly, informants with differing demographics may have differing experiences and may therefore provide different information.

\subsection{Collecting information from informants: research strategies}

Having defined situations, research models, informants and their characteristics, and types of information, we now consider how information is collected from informants. We consider three of the main research strategies in empirical software engineering for collecting information, i.e., the case study, the survey study and the interview study. We recognise that there are other research strategies for collecting information from practitioners, e.g., action research, ethnography, and grey literature reviews. To retain the focus of this paper, we focus on a subset of possible research strategies. Future research could extend this work to include the other strategies. We are also aware of research methods, such as focus group, questionnaire and document analyses. These methods can be used in different permutations in the strategies. Again, to retain the focus of this paper, we do not consider these methods in the current paper.

Figure \ref{fig:case-design-v4}, Figure \ref{fig:survey-design-v4} and Figure \ref{fig:interview-design-v4} relate situations, informants and research models to case study, survey study and interview study respectively. Table \ref{table:compare-research-strategies-v04} provides a comparison of the three research strategies in relation to the framework.

\subsubsection{Case study} 

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{images/case_study_design_v5.png}
    \caption{Design of case study. Information is collected from informants about situation S\textsubscript{1}. Informants who are actors undertake activities in the situation. Informants who are observers observe the situation, e.g. observe actors undertaking activities. Advisors are external to the situation but have relevant information for the research.}
    \label{fig:case-design-v4}
\end{figure}

In a case study, the researcher focuses on one (or sometimes more than one) specific situation in its natural environment and studies that situation intensively~\cite{runeson2009guidelines}. The researcher works with some kind of research model, however formally or informally developed, and makes inferences (e.g., inductively, abductively, or deductively) between the specific situation and the model. Because the researcher works with a specific situation, the researcher is much better able to identify practitioners that are relevant to that situation and to the research model, and to then evaluate whether a practitioner is suitable as an informant about that situation; and also the researcher is better able to determine the suitable \emph{role} of informant for that practitioner. The researcher is also better able to control the types of information collected, i.e., empirical information about the situation, theoretical information, or both. Finally, the researcher is able to use methods of triangulation across multiple sources of information, e.g., across informants, project documentation, emails,to get a better `handle' on the situation and to better assure the validity and relevance of information in relation to the research model.

\subsubsection{Interview study} 

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{images/survey_study_design_v5.png}
    \caption{Design of survey study. Information is collected from informants but the situations, S\textsubscript{n} through S\textsubscript{n+m}, are at--best partially known and therefore the number of situations, as well as the relationships between the informants and the situations, is not easy to determine.}
    \label{fig:survey-design-v4}
\end{figure}

In an interview study, the researcher typically focuses on collecting information from multiple practitioners who each have experience of one or more situations. This is like the survey study however the researcher has more control over the recruitment of who to interview, and also has more control over the information that can be collected, because of the interaction possible in the interview. Some consequences are that the researcher is, at least in principle, able to influence which situation or situations the informant refers to, is able to know more about the situations of interest (because they can gather more information on the situation/s experienced by the informant), can better determine the \emph{role} of the informant, and can influence the types of information provided by the informant.

\subsubsection{Survey study} 

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{images/interview_study_design_v4.png}
    \caption{Design of interview study. Information is collected from informants where the situations, S\textsubscript{n} through S\textsubscript{n+m}, can be better known by the researcher and therefore the number of situations, as well as the relationships between the informants and the situations, is relatively well known.}
    \label{fig:interview-design-v4}
\end{figure}

In a survey, the researcher typically focuses on collecting information from multiple practitioners who have experience of situations where those situations are, \emph{at best}, only partially known to the researcher.

Again, the researcher works with some kind of research model, however formally or informally developed, and again the researcher makes inferences. Because the researcher does not work with known situations (indeed has little control on the selection of situations), the researcher is much less able to identify appropriate practitioners, less able to evaluate whether a practitioner is suitable as an informant for their research; and also the researcher is less able to determine the suitable \emph{role} of informant for that practitioner. It is also much harder for the researcher to determine whether the practitioner is providing information based on one specific situation, or some accumulation of multiple situations. And it is harder for the researcher to control the types of information collected, i.e., empirical information about the situation, theoretical information, or some mixture of both. Finally, it is much harder to triangulate information to get a `handle' on the phenomena of interest. We refer to phenomena here because it is not clear what constitutes the situation.

Instead, and broadly speaking, the researcher relies on statistical analyses of the responses to the survey.

For surveys, one research--design decision a researcher might make is to ask the informant to respond to the survey on the basis of one specific situation that the informant has experienced. Another research--design decision is to ask the informant to provide a description of the situation. A third research--design decision is to seek several practitioners to provide information about the same situation, for triangulation, though this decision also raises potential challenges in double--counting responses.

% \clearpage

\begin{table*}[htp]
    \small
    \caption{A comparison of research strategies in relation to components of the framework.}
    \label{table:compare-research-strategies-v04}
    \centering
    \begin{tabular}{| p{3.6cm} | c |  c | c | }
        \toprule
        \textbf{Property} & \textbf{Case Study} & \textbf{Interview Study} & \textbf{Survey Study}\\
        \midrule
        % \hline
        % \hline
        \multicolumn{4}{| l |}{\emph{Situations}}\\
        % \hline
        \midrule
        Explicitness of source situation/s & Explicit & Explicit & Implied \\
        % \hline
        \midrule
        Level of abstraction & Variable & Stable \\
        % \hline
        \midrule
        Number of situations studied & 1 or Few & Variable & Unknown \\
        % \hline
        \midrule
        \multicolumn{4}{| l |}{\emph{Informants}}\\
        \hline
        Direct access to candidates & Good & Some & None\\
        % \hline
        \midrule
        Number of informants & Some & Some & Many \\
        % \hline
        \midrule
        Number of informants per situation & Some & 1 or Some & 1  \\
        % \hline
        \midrule
        Ability to identify informants & Easier & Easier & Harder \\
        % \hline
        \midrule
        Ability to evaluate informants & Easier & Easier & Harder x\\
        % \hline
        \midrule
        Ability to control types of information & Easier & Easier & Harder \\
        % \hline
        \midrule
        \multicolumn{4}{|l|}{\emph{Types of information}}\\
        % \hline
        \midrule
        Restrict to description & Easier & Easier & Harder\\
        % \hline
        \midrule
        Restrict to opinion & Easier & Easier & Easier\\
        % \hline
        \midrule
        \multicolumn{4}{|l|}{\emph{Inference to research model}}\\
        % \hline
        \midrule
        Focus of information validation & Within situation & Across responses & Across responses\\
        % \hline
        \midrule
        Method of information validation & Triangulation & Statistical & Statistical\\ 
        % \hline
        \midrule
        Method of generalisation & Analytical & Analytical & Statistical\\
        \bottomrule
    \end{tabular}
\end{table*}

==> x_archive/X_thoughts.tex <==
\clearpage
\section*{Thoughts}
\textcolor{magenta}{Note:} This section is to raise questions, comments about what might go into the paper, or not etc.
\begin{enumerate}
    \item To reduce the size of the paper, we might simplify the framework (e.g. remove figures) and/or the checklist, or possibly remove the checklist (?)
    \item If we did snowballing, or some kind of systematic review, why are we doing it? An SR of some kind might: 
    \begin{enumerate}
        \item Give us information on frequency/prevalence e.g., how much the problem we have identified is \textit{not} considered in research. We can however already argue from the guidelines, i.e., the guidelines haven't identified it.
        \item Give us `false negatives' (a bit like the Singer paper) where we see that researchers are doing what we are talking about, but what they are doing is not recognised in the guidelines.
        \item Give us information on \textbf{the way that researchers talk about participant recruitment and whether and how they talk about threats based on that recruitment}.
    \end{enumerate} 
    \item In the absence of an SR we might select some notable papers (e.g., highly cited papers, or Paper Award papers) and compare those with the framework/checklist?
    \item We might look at other guidelines, e.g., Kitchenham et al.'s Preliminary Guidelines, Guidelines on Focus Groups, the Empirical Standards being pushed. This would be a way of complementing the comparison of the Guidelines papers and would allow us to show that, from different perspectives (different authors, different research methods, different aspects of research, like sampling) researchers have `missed' this issue. 
    \item In Section X3
    I have introduced illustrative examples. I was thinking of something different to our three exemplar papers and the illustrative examples might provide a good way to talk about the issue/s early in the paper, without making judgments on the illustrative example papers themselves. We might use the examples again later in the paper as a complement to the exemplars and the guidelines; or we might not.
    % \item Given the inclusion of a reference example for case studies, should we include a reference example for interviews and for surveys? Promising examples might be: \cite{SCHERMANN201841} because they report two interview studies and a survey study; and \cite{KROEGER2014252} because they provide detail on the companies and participants (though not the recruitment process).
\end{enumerate}


==> x_archive/Y_additional_material.tex <==
\clearpage
\section*{Additional material}

\subsection{Participants as research instruments}
%\label{subsection:participants-as-research-instruments}
Our interest is in information that participants can provide about events external to the participant, e.g., about the behaviour of software phenomena that they observe. We can \textit{model} a participant as a kind of research instrument, or in D'Andrade's \cite{dandrade1974memory} term, as a `behaviourscope'. We can then think of the participant in terms of: their reliability (how consistently they observe the world) and their validity (how accurately they observe the world); in terms of bias; and in terms of information accuracy.

\subsubsection{Validity and reliability}

Homburg et al. \cite{homburg2012drives} used data from 127 studies across six major marketing and management journals to investigate hypotheses concerning key--informant's reliability and validity in survey studies. Unfortunately, Homburg et al. do not define what they mean by \textit{key informant}. Phillips \cite{phillips1981assessing}, cited by Homburg et al. \cite{homburg2012drives} explain that informants are chosen because they have special qualifications such as particular status, specialized knowledge, or even accessibility to the researcher. We discuss key informants later in this section.

Homburg et al. \cite{homburg2012drives} draw on social cognition theory to identify two concepts central to their research: (1) availability of relevant information and (2) difficulty of retrieval. The availability of relevant information and the difficulty of retrieval of information introduce random error. But they can also introduce systematic error. Where an informant lacks pertinent information or struggles to retrieve such information, these informants may provide a random best guess (thus threatening reliability) or may use some heuristic to guide their response (thus threatening validity).

Relating this to the model in Figure \ref{figure:generalised-karlstrom-and-runeson-figure}:

\begin{enumerate}
    \item For case studies, such as the Karlstr{\"o}m and Runeson \cite{karlstrom2006integrating} reference example, we can have more confidence (in relative terms) that the participants will have relevant information as the participants are part of the cases being studied. Note that there may still be systematic error, e.g., from cultural beliefs present within the respective cases being studied.
    
    \item In interview studies (e.g., \cite{curtis1988field}), we can have more confidence (in relative terms) that the participants will have relevant information as the participants have some relationship with the cases of interest. There may still be systematic error, though the content of that error may be different.

    \item It surveys, it is uncertain as to whether the participants have access to relevant information.
    
\end{enumerate}

For reliability, Homburg et al. \cite{homburg2012drives} propose five sets of factors affecting reliability: (1) construct characteristics, (2) informant characteristics, (3) organizational characteristics, and (4) industry characteristics. Because we also investigate formal considerations, we consider method characteristics as a fifth set. For validity, Homburg et al. \cite{homburg2012drives} focus on their construct characteristics.  A summary of their results are presented in Table \ref{table:homburg-hypotheses}.

\begin{table}[!ht]
    \small
    \caption{Constructs affecting reliability and validity (from  \cite{homburg2012drives})}
    \label{table:homburg-hypotheses}
    \centering
    \begin{tabular}{| p{0.5cm} | p{6.6cm} | }
        \hline
        \textbf{\#} & \textbf{Hypothesis}\\
        \hline
        \hline
        \multicolumn{2}{| l |}{Impact of constructs characteristics on \textbf{reliability}}\\
        H1 & The reliability of key informant responses is greater for constructs pertaining to the present (vs. the past).\\
        H2 & The reliability of key informant responses is greater for objective constructs (vs. more subjective constructs)\\
        H3 & The reliability of key informant responses is greater for constructs pertaining to more salient events (vs. more routine events).\\
        
        \multicolumn{2}{| l |}{Impact of informant characteristics on \textbf{reliability}}\\
        H6 & The reliability of key informant responses is greater for informants in higher hierarchical positions (vs. lower hierarchical positions).\\
        
        \multicolumn{2}{| l |}{Impact of method characteristics on \textbf{reliability}}\\
        H14 & Key informant reliability estimates will be greater if triangulation is conducted using archival data (vs. survey data).\\
        
        \multicolumn{2}{| l |}{Impact of construct characteristics on \textbf{validity}}\\
        H16 & The validity of key informant responses is greater for constructs pertaining to the present (vs. the past).\\
        H17 & The validity of key informant responses is greater for objective constructs (vs. more subjective constructs)\\
        H18 & The validity of key informant responses is greater for constructs pertaining to more salient events (vs. more routine events).\\
  
        \hline
    \end{tabular}
\end{table}


\subsubsection{Bias}

Mohanani et al. \cite{mohanani2018cognitive} report a systematic mapping study of cognitive biases in software engineering. Chattopadhyay et al. \cite{chattopadhyay2020tale} report a two--part field of the presence of cognitive biases in software development, drawing on the work of Mohanani et al. \cite{mohanani2018cognitive}. Mohanani et al. cite Flesichmann et al.'s \cite{fleischmann2014cognitive} work.


\begin{table}[!ht]
    \small
    \caption{Cognitive bias (\cite{mohanani2018cognitive}, see also \cite{fleischmann2014cognitive}}
    %\label{table:cognitive-biase}
    \centering
    \begin{tabular}{| p{0.5cm} | p{1cm} | p{5.4cm} | }
        \hline
        \textbf{\#} & \textbf{Bias} & \textbf{Description}\\
        \hline
        \hline
        1  & Stability & Biases that lead individuals to persevere with established or familiar options despite the presence of superior information, arguments or conditions.\\
        2  & Action--oriented & Biases that lead individuals to premature decisions without considering relevant information or alternative courses of action.\\
        3 & Pattern--recognition & Biases that lead individuals to attend more to information that is familiar.\\
        4 & Perception & Biases that prejudice the processing of new information.\\
        5 & Memory & Biases that affect recall of information or experience.\\
        \hline
    \end{tabular}
\end{table}

\subsubsection{Information accuracy}

Bernard et al. \cite{bernard1984problem} are concerned with the validity and accuracy of the ``naive senses'' of informants.  They review previous work in three areas: recall of child care behavior; recall of health seeking behavior; and recall of communication and social interactions. They identify a number of concerns with the use of informants. As an illustrative example, we quote their summary of a study by Kornfield: ``Informants showed much higher agreement about what waiters were wearing than about what waitresses were wearing, despite the fact that none of the restaurants in question had waiters. Informants provided greater detail about the kind of music that was playing in restaurants that, in fact, did not have music than they provided for restaurants that did have music.'' (\cite{bernard1984problem}, p. 509)

We summarise Bernard et al.'s \cite{bernard1984problem} more relevant concerns here:
\begin{enumerate}
    \item Informants \textit{are} inaccurate; memory \textit{does} decay exponentially with time.
    \item There appears to be systematic distortion in how informants recall just about everything.
    \item Recall may be effected by the subject of the study, by whether informants are aided in their recall in some way during the interview, by whether they keep diaries, by conditions of the interview, or by a variety of cultural factors.
    \item If informants agree with one another in information that they independently provide, then there must be a basis for this. The two likely explanations are norms and actual experience.
    \begin{enumerate}
        \item When informants don't recall an actual experience, they are more likely to rely on a cultural norm for their answer.
        \item Informants who have an actual experience are more likely to resist badgering (are less likely to `back down'). A consequence is that answers that show more resistance to badgering is more likely to be accurate.
    \end{enumerate}
    \item Knowing which informants are likely to be least accurate is surely important; but knowing whether \textit{any} informant is sufficiently accurate to rely upon his or her responses is more important still.
    \item Interviewing many inaccurate informants will not solve the accuracy/validity problem
\end{enumerate}

Bernard et al.'s \cite{bernard1984problem}'s observation about cultural norms is demonstrably present in software engineering. For example, Rainer et al. \cite{rainer2003persuading} found that practitioners prefer local opinion over other sources of knowledge. Devanbu et al. \cite{devanbu2016belief} conducted a large survey of Microsoft employees (n=564) finding that developers beliefs are based primarily on their personal experience and then, second, on their peers' opinions. (By contrast, research papers were ranked fifth out of six.)

\subsection{Key informants}

Marshall \cite{marshall1996key} defines a key informant as an expert source of information. He identifies five characteristics of ideal key informants as well as strengths and weaknesses. These are all summarised in Table \ref{table:key-informants}.

In software engineering research, an example of the use of key informants would be an expert panel, e.g., \cite{li2003ranking}.

\begin{table}[!ht]
    \small
    \caption{Characteristics of ideal key informants, and strengths and weaknesses (from \cite{marshall1996key}}
    %\label{table:key-informants}
    \centering
    \begin{tabular}{| l | p{7cm} | }
        \hline
        \textbf{\#} & \textbf{Description}\\
        \hline
        \hline
        \multicolumn{2}{|l|}{Characteristics}\\
        C1 & \textbf{Role in community}. Their formal role should expose them to the kind of information being sought by the researcher\\
        C2 & \textbf{Knowledge}. In addition to having access to the information desired, the informant should have absorbed the information meaningfully.\\
        C3 & \textbf{Willingness}. The informant should be willing to communicate their knowledge to the interviewer and to cooperate as fully as possible.\\
        C4 & \textbf{Communicability}. They should be able to communicate their knowledge in a manner that is intelligible to the interviewer.\\
        C5 & \textbf{Impartiality}. Key informants should be objective and unbiased. Any relevant biases should be known to the interviewer\\
        \hline
        \multicolumn{2}{|l|}{Advantages}\\
        A1 & Quality of data that can be obtained in a relatively short period of time. To obtain the same amount of information and insight from in-depth interviews with other members of a community can be prohibitively time-consuming and expensive\\
        \hline
        \multicolumn{2}{|l|}{Disadvantages}\\
        D1 & Unlikely to represent, or even understand, the majority view of those individuals in their community.\\
        D2 & The identification of key informants may be in error because some societies may attract people who wish to improve their status but do not have the necessary skills of a true key informant\\
        D3 & Informants are different to informers, who are more likely to be biased and to have their own agenda.\\
        D4 & Key informants might only divulge information that is politically acceptable and social rules could discourage the researcher from publishing potentially sensitive data which may be ascribed to a particular informant.\\
        \hline
    \end{tabular}
\end{table}

% \subsection{Relevant knowledge}
% In this subsection we draw on Devanbu et al., Rainer et al., Hoda's paper on recruiting participants to talk about relevant knowledge.

\subsection{Summary}

We need more credible participants for our studies, i.e., informants who are more reliable and who can provide more valid information. Such information is the foundation of empirical work that relies on practitioners, e.g., interviews, focus groups, surveys. `Input' information from practitioners that is invalid, or information for which its validity is highly uncertain, fundamentally undermines the validity of our subsequent research findings, regardless of the reliability of the research process. (Essentially, we have Garbage In, Garbage Out.) Rephrasing Bernard et al. \cite{bernard1984problem}, many studies all reporting invalid findings will not solve the problem. 

Treating the recruitment of participants as a matter of better sampling, so as to `produce' a more representative sample, is potentially mis--framing the problem. This is because participants are often not the target population. In our studies, we are often interested in what participants can tell us \textit{about} our target population, e.g., what an informant tells us about requirements engineering, or software testing, or software projects, or defects.

As a step toward addressing these concerns, we propose a framework and checklist to help researchers think about the recruitment of credible participants.

==> x_comments.tex <==
% Uncertainty about the credibility of participants in an empirical study threatens the reliability, validity and relevance of the research. If we do not have confidence that we are collecting data from credible participants (credible for that study), on what basis can we have confidence in the validity of the information those participants provide to the researcher? Such threats affect all research methods that collect data from participants, and therefore may affect the results of already--completed empirical studies as well as many potential studies in the future.

   % \item If informants agree with one another in information that they independently provide, then the two likely explanations are \emph{norms} and \emph{actual experience}.
    % \begin{enumerate}
    %     \item When informants do not recall an actual experience, they are more likely to rely on a cultural norms for their answer.
    %     \item Informants who have an actual experience are more likely to resist badgering (are less likely to ``back down''). A consequence is that answers that show more resistance to badgering are more likely to be accurate.
    % \end{enumerate}
    % \item Knowing which informants are likely to be least accurate is important. But knowing whether \emph{any} informant is sufficiently accurate is more important.
    
% \subsection{The participant as a research instrument}
% \label{subsection:participants-as-research-instruments}

% We can \emph{model} a participant as a kind of research instrument, or in D'Andrade's \cite{dandrade1974memory} term, as a `behaviourscope'. Bernard et al.~\cite{bernard1984problem} write, ``It is not enough to point out that there are reasons for the fact that informants are poor instruments for studying human behavior. We must begin a systematic effort to discover, for each kind of data
% that we want, what the error bounds are for the instruments that we use to
% collect those data.''

% We can then think of the participant in terms of their reliability (how consistently they observe the world), their validity (how accurately they observe the world) and their relevance (how relevant their observations are to the research); in terms of bias; and in terms of information accuracy. We briefly consider each of these below.

% As noted in Section~\ref{section:introduction}, we are interested in what participants can say about software engineering phenomena they perform or observe, e.g., about software inspections or pair programming or cost estimation. In these situations, the item of interest is the phenomenon external to the participant. The participant is not the item of interest. Figuratively, the participant acts as a lens through which the researcher can observe the item of interest. A case study can illustrate this clearly, e.g., participants are interviewed for their observations of the item of interest, i.e., the case. Discussions about a sample of participants, and whether and how representative that sample may be, can therefore sometimes be misleading. We consider it helpful to also reason in terms of whether the sampled participants can provide information on a representative sample of external phenomena. 

% This issue -- of the relationship of the participant to the item of interest -- does not seem to be explicitly discussed in the software engineering research literature. For case studies, the relationship appears self--evident but even there the relationship may be more complicated than assumed. For empirical studies more generally, and not just case study, there seems to be an unstated assumption, or assumptions, about the relationship between participants and items of interest (or, alternatively phrased, of units of study, or of cases). Possible assumptions might be (these are not exhaustive):
% \begin{itemize}
%     \item That a sufficient number and/or diversity of participants provides information on a sufficient number and/or diversity of items of interest.
%     \item That a sufficiently `random' number of participants provides information on a sufficiently `random' number of items of interest.
%     \item That each participant represents one item of interest.
%     \item That if the study recruits `enough' participants, the study will be able to investigate `enough' items of interest.
% \end{itemize}

% \emph{Case study:} Research guidelines for conducting case study research within software engineering were first published as a checklist, by Höst and Runeson~\cite{host2007checklists}, at a conference in 2007. Runeson and Höst then published a more extensive set of guidelines as a journal article in 2009~\cite{runeson2009guidelines} and then as a book~\cite{runeson2012book} in 2012. Verner et al.~\cite{verner2009guidelines} published guidelines for industrial case studies in software engineering at a conference in 2009.

% \emph{Interview study:} We did not find guidelines for interview study in software engineering that are comparable to the case study guidelines or to the survey study guidelines (discussed next). We therefore had to relax our requirement for post--2009 publication for these interview ``guidelines'' and we also chose two articles. The first article, by Strandberg~\cite{Strandberg2019}, provides advice concerning ethics in interview studies. The second article, by Hove and Anda~\cite{hove2005experiences}, shares their experiences of conducting interview studies in software engineering.

% \emph{Survey:} Empirically evaluated survey guidelines are published by Molléri et al.~\cite{molleri2020empirically} in 2020. Their article synthesises a range of previous guidelines on survey studies, e.g.,~\cite{molleri2019cerse,molleri2016survey}.

% \emph{Participant recruitment:} Salleh et al.'s~\cite{salleh2018recruitment} article does not present \emph{guidelines} but rather, in a way that is similar to Hove and Anda~\cite{hove2005experiences}, shares their experience of conducting interviews. Salleh et al.'s~\cite{salleh2018recruitment} experience is of conducting research in industrial contexts.

% We looked at the guidelines for using focus groups proposed by Kontio et al.~\cite{kontio2008focus} and published in 2008. Furthermore, we reviewed the preliminary guidelines for empirical research proposed by Kitchenham et al.~\cite{kitchenham02guidelines} and published in 2002. Moreover, we consider the guidelines for ethnographic studies by Zhang et al.~\cite{zhang2019ethnographic}, published in 2019. Finally, we also looked at the empirical standards being developed in conjunction with ACM SIGSOFT~\cite{ACM20} and published in 2021.

% We then shortlisted articles presenting empirical studies published before 2009, since 2009 is the year that both Runeson and H{\"o}st~\cite{runeson2009guidelines} and Verner et al.~\cite{verner2009guidelines} published their guidelines on case study research in SE; also, guidelines for surveys were published after that date. We shortlisted some articles as `negative examples', e.g., we wanted to know whether the already--published article would present any problems for future application of the framework. Other articles we shortlisted as `positive examples'. We decided to only include empirical studies published before 2009 to control for the potential influence of guidelines.

% \sout{To demonstrate the use of the framework, a selection of previously published primary studies was conducted.} To select primary studies for demonstration, both authors independently searched for candidate articles to consider. Searches were primarily undertaken using Google Scholar \textcolor{magenta}{(again, we do not need to use multiple search engines because we are not undertaking an exhaustive search)}, and highly cited articles were prioritised, based on the assumption that they were more likely to have valuable information. Furthermore, we prioritised articles having good descriptions of the participants in the studies. The candidate articles were then read independently by both authors and discussed in online meetings, with the final selection made on the basis of unanimous agreement.

% We shortlisted articles presenting empirical studies published before 2009, since 2009 is the year that both Runeson and H{\"o}st~\cite{runeson2009guidelines} and Verner et al.~\cite{verner2009guidelines} published their guidelines on case study research in SE; also, guidelines for surveys were published after that date. We shortlisted some articles as `negative examples', e.g., we wanted to know whether the already--published article would present any problems for future application of the framework. Other articles we shortlisted as `positive examples'. We decided to only include empirical studies published before 2009 to control for the potential influence of guidelines.

% \austen{I am wondering whether we might remove Table \ref{table:assessment-of-framework}, to save space, and instead list the three references and then point the reader to Table~\ref{table:compare-exemplars-with-framework}.} \claes{The table does not take that much space, and some people find it positive to not only have a flow of text. I suggest keeping it.}

% In this section, we compare our framework against published guidelines, checklists and papers providing guidance based on experience within software engineering. 

% \claes{I strongly believe that we need to have our method section before this section. This is part of how we approached it, or now claim that we did. Furthermore, I do not think it is a matter of comparing. It is more reviewing the guidelines with a lens focusing on what the guidelines state concerning participants.}

%\subsection{Case study}
%\label{section:casestudy}

% \subsection{Guidelines for ethnographic studies}
% 
% \textcolor{magenta}{Zhang et al.~\cite{zhang2019ethnographic} present a critical review and checklist for conducting ethnographic studies in software engineering. An ethnographic study is a different kind of empirical study to an interview study or a survey study because the ethnographic study directly observes the practitioners. As with Salleh et al.'s~\cite{salleh2018recruitment} discussion of participant recruitment, we are interested in whether the guidelines for ethnographic studies consider the credibility of the practitioners being observed.}

% \textcolor{magenta}{Zhang et al.~\cite{zhang2019ethnographic} organise their checklist into three sections: design, execution and reporting. Their checklist recognises practitioners (e.g., the checklist asks, `State the \emph{key person} (e.g., Project Leader, DevOps Consultant) you [are] studying in the organization and explain the relationship between you and him/her.') but does not provide guidance on how to assess the credibility of the practitioners being studied. As with other guidelines, Zhang et al.'s~\cite{zhang2019ethnographic} checklist does not address the items being identified in the framework.}

%\subsection{Other guidelines}
%\label{section:other-guidelines}

%In principle, more recent guidelines ought to be a superset of the \emph{better} preceding guidelines. An implication is that there should not be the need to compare our framework with guidelines published \emph{before} the case study and survey study guidelines, or before the guidance papers, that we discuss in Section~\ref{section:reviewingguidelines}. On the other hand, there may be more recent guidelines that synthesise the case study and survey study guidelines, and the experiences reported concerning interview studies. 

%Given the insights arising from our comparisons -- essentially, that the framework focuses on characteristics that have not been considered in neither the guidelines nor the articles reporting experiences -- we looked at two sets of guidelines that precede the case study and survey study guidelines, and also at two  more recent `guidelines' that succeed the case study and survey study guidelines.  

%Interestingly, the three reference examples discussed in Section~\ref{section:reference-examples} include more details about the participants, and their recruitment, in the respective study than are advised by the guidelines. Thus, several authors acknowledge the importance of describing the characteristics of participants and the importance of recruiting the `right' participants. On the basis of our review of three reference examples and of a selection of guidelines, it appears, unfortunately, that the guidelines do not address the challenges of recruiting credible practitioners. We therefore argue that the framework complements and extends existing guidelines by recognising characteristics that should be considered by researchers to recruit credible practitioners for their empirical studies.

% In summary, it means that the initial guidelines are quite ``light'' concerning participant recruitment.

%\subsection{Summary of advice on the selection of participants}

% \claes{How about having this in the end of Section 5? The framework needs to be described before being compared with the guidelines.}

% \begin{table*}[htp]
%     \small
%     \caption{Comparison of framework with guidelines}
%     \label{table:compare-guidelines-with-framework}
%     \centering
%     \begin{tabular}{| l || l || c | c | c || c | c | c | c | c | c || c | c | }
%         \toprule
%         %  & \textbf{Rl} & \textbf{Rlvnt} & \textbf{Rcnt} \multicolumn{2}{| c ||}{\textbf{Info.}} & \multicolumn{6}{| c |}{\textbf{Quality}}\\
        
%         & \textbf{Role} & \multicolumn{3}{ c ||}{\textbf{R\textsuperscript{3} model}} & \multicolumn{6}{ c ||}{\textbf{Quality}} & \multicolumn{2}{ c |}{\textbf{Info.}}\\
        
%         Paper & \textbf{POA} & \textbf{Real} & \textbf{Rlvnt} & \textbf{Rcnt} & \textbf{E} & \textbf{P}  & \textbf{S} & \textbf{R} & \textbf{W} & \textbf{D} & \textbf{Fact} & \textbf{Blfs} \\
%         \midrule
%         \multicolumn{13}{| l |}{Compare framework against guidelines}\\
%         4 \cite{runeson2009guidelines} & & & & & & & & & & & & \\
%         5a \cite{Strandberg2019} & & & & & & & & & & & & \\
%         5b \cite{hove2005experiences} & & & & & & & & & & & &\\
%         6 \cite{molleri2020empirically} & & & & & & & & & & & &\\
%         7 \cite{salleh2018recruitment} & & & & & & & & & & &  &\\
%         \midrule
%         \multicolumn{13}{| l |}{Further comparison of framework against guidelines}\\
%         8 \cite{kontio2008focus} & & & & & & & & & & & &\\
%         9 \cite{kitchenham02guidelines} & & & & & & & & & & & &\\
%         10 \cite{zhang2019ethnographic} & & & & & & & & & & &  &\\
%         11 \cite{ACM20} & & & & & & & & & & & &\\
%         \bottomrule
        
%         % \midrule
        
%         % Performer & YES & YES & YES & \multicolumn{6}{c ||}{\dots} & YES & YES \\
%         % Observer & YES & yes & yes & \multicolumn{6}{c ||}{\dots} & yes & yes\\
%         % Advisor & yes & maybe & maybe & \multicolumn{6}{c ||}{\dots} & -- & yes\\
%         % \bottomrule
%         % \multicolumn{12}{l}{Notes for R\textsuperscript{3} model:}\\
%         % \multicolumn{12}{l}{YES=strongly meets criterion.}\\
%         % \multicolumn{12}{l}{yes=moderately meets criterion.}\\
%         % \multicolumn{12}{l}{maybe=may meet criterion depending on context.}\\
%         % \multicolumn{12}{l}{Notes for Information:}\\
%         % \multicolumn{12}{l}{YES = more likely to provide}\\
%         % \multicolumn{12}{l}{yes = may be able to provide}\\
%         % \multicolumn{12}{l}{-- = cannot provide facts about the item/s of interest}\\
%         % \multicolumn{12}{l}{We intentionally do not populate the Quality criteria.}\\
%     \end{tabular}
% \end{table*}

% \begin{table*}[htp]
%     \small
%     \caption{Verbatim extracts from guidelines and checklist papers.}
%     \label{table:extracts-from-guidelines}
%     \centering
%     \begin{tabular}{| l | p{13cm} |}
%         \toprule
%         \textbf{Ref.} & \textbf{Extract}\\
%         \multicolumn{2}{| l |}{Guidelines and recommendations on the selection of participants}\\
%         \cite{runeson2009guidelines} & - Is the case adequately defined (size, domain, process, \textbf{subjects}...)?\\
%         & - Is there a rationale behind the selection of \textbf{subjects}, roles,\dots etc.?\\
%         % & & 13. & Are measurement instruments and procedures well defined (measurement definitions, interview questions)?\\
%         \cite{Strandberg2019} & \\
%         \cite{hove2005experiences} &\\
%         \cite{molleri2020empirically} & - Is the population or the survey's target audience characterized (e.g., through audience analysis)?\\
%         & - Is the kind of sample (i.e., probabilistic, non-probabilistic) defined?\\
%         & - Is the sampling process described\dots?\\
%         & - Are the sources of sampling\dots defined?\\
%         & - Are the strategies and criteria to select units (of observation, of analysis and search unit) stated?\\
%         %& & 5C & Are the \textbf{demographic} questions formulated according to the audience?\\
%         \cite{salleh2018recruitment} &\\
%         \midrule
%         \multicolumn{2}{| l |}{Additional advisory sources on the selection of participants}\\
%         \cite{kontio2008focus} & \\
%         \cite{kitchenham02guidelines} &\\
%         \cite{zhang2019ethnographic} &\\
%         \cite{ACM20} &\\
        
%         \midrule
%         \bottomrule
%     \end{tabular}
% \end{table*}

% \subsection*{Leftovers}
% \austen{I am not sure yet whether/where/how to retain these in the paper}

% \claes{Personally, I like Table 6. It contrast some common research approaches when the framework is useful.}

% \subsubsection*{Comparison table}

% Table \ref{table:compare-research-strategies-v04} provides a summary comparison of the three research strategies in relation to the framework.

% \begin{table*}[htp]
%     \small
%     \caption{A comparison of research strategies in relation to components of the framework.}
%     \label{table:compare-research-strategies-v04}
%     \centering
%     \begin{tabular}{| p{3.6cm} | c |  c | c | }
%         \toprule
%         \textbf{Property} & \textbf{Case Study} & \textbf{Interview Study} & \textbf{Survey Study}\\
%         \midrule
%         % \hline
%         % \hline
%         \multicolumn{4}{| l |}{\emph{Situations}}\\
%         % \hline
%         \midrule
%         Explicitness of source situation/s & Explicit & Explicit & Implied \\
%         % \hline
%         \midrule
%         Level of abstraction & Variable & Consistent & Unknown\\
%         % \hline
%         \midrule
%         Number of situations studied & 1 or Few & Variable & Unknown \\
%         % \hline
%         \midrule
%         \multicolumn{4}{| l |}{\emph{Participants}}\\
%         \hline
%         Direct access to candidates & Good & Good & Limited\\
%         % \hline
%         \midrule
%         Number of participants & Some & Some to many & Many \\
%         % \hline
%         \midrule
%         Number of participants per situation & Some & 1 or Some & 1  \\
%         % \hline
%         \midrule
%         Ability to select practitioners & Easier & Easier & Harder \\
%         % \hline
%         \midrule
%         Ability to evaluate practitioners & Easier & Easier & Harder\\
%         % \hline
%         \midrule
%         Ability to control types of information & Easier & Easier & Harder \\
%         % \hline
%         \midrule
%         \multicolumn{4}{|l|}{\emph{Types of information}}\\
%         % \hline
%         \midrule
%         Restrict to description & Easier & Easier & Harder\\
%         % \hline
%         \midrule
%         Restrict to belief & Easier & Easier & Harder\\
%         % \hline
%         \midrule
%         \multicolumn{4}{|l|}{\emph{Inference to research model}}\\
%         % \hline
%         \midrule
%         Focus of information validation & Within situation & Across responses & Across responses\\
%         % \hline
%         \midrule
%         Method of information validation & Triangulation & Replication & Statistical\\ 
%         % \hline
%         \midrule
%         Method of generalisation & Analytical & Analytical & Statistical\\
%         \bottomrule
%     \end{tabular}
% \end{table*}

% \subsubsection*{Research strategies for collecting information from participants}

% In a case study, the researcher focuses on one (or sometimes more than one) specific situation in its natural environment and studies that situation intensively~\cite{runeson2009guidelines}. The researcher works with some kind of research model, however formally or informally developed, and makes inferences (e.g., inductively, abductively, or deductively) between the specific situation and the model. Because the researcher works with a specific situation, the researcher is much better able to identify practitioners that align with the research model, is better able to determine the suitable \emph{role} of the practitioner, is better able to assess the quality of information the practitioner might provide (cf. Table~\ref{table:summary-of-framework}), and can therefore better evaluate whether each practitioner is suitable as a credible participant. The researcher is also better able to control the types of information collected, i.e., to collect facts about the world or beliefs about the world, or both. Finally, the researcher is able to use methods of triangulation across multiple sources of information, e.g., across participants, project documentation, emails,to get a better `handle' on the situation and to better assure the validity and relevance of information in relation to the research model.

% In an interview study, the researcher typically focuses on collecting information from multiple practitioners who each have experience of one or more situations. Again, the researcher works with some kind of research model etc. Because the researcher typically has direct contact with the prospective participants, as part of the recruitment process, the researcher has the opportunity to identify practitioners that align with the research model, is better able to determine the suitable \emph{role} of the practitioner, is better able to assess the quality of information the practitioner might provide (cf. Table~\ref{table:summary-of-framework}), and can therefore better evaluate whether each practitioner is suitable as a credible participant. The researcher is also better able to control the types of information collected, i.e., to collect facts about the world or beliefs about the world, or both. Unlike the case study, however, the researcher is less likely to be able to draw on triangulation as a approach to quality assurance of the information collected from the participants.

% In a survey, the researcher typically focuses on collecting information from multiple practitioners who have experience of situations where those situations are, \emph{at best}, only partially known to the researcher. Again, the researcher works with some kind of research model etc. Because the researcher has limited control on the recruitment process, the researcher lacks the opportunity to identify practitioners that align with the research model, is not able to determine the suitable \emph{role} of the practitioner, is not able to assess the quality of information the practitioner might provide (cf. Table~\ref{table:summary-of-framework}), and therefore has limited opportunity to evaluate whether each practitioner is suitable as a credible participant. The researcher also has limited control on the types of information the participant provides, i.e., whether the participant reports facts about the world or beliefs, or both or neither. The researcher is also not able to draw on triangulation as a approach to quality assurance of the information collected from the participants.

% There are several survey--study designs available to the researcher. For example, the researcher might ask the participant to respond to the survey on the basis of one specific situation that the participant has experienced, ask the participant to provide a description of the situation, or to ask several practitioners to provide information about the same situation (offering a kind of triangulation). With all these designs, there remain challenges in assuring the recruitment of appropriately credible participants.

% Table~\ref{table:compare-Freimut-with-framework-part-1} and Table~\ref{table:compare-Freimut-with-framework-part-2} show how the Freimut et al.~\cite{freimut05} article maps to the framework. With Table~\ref{table:compare-Freimut-with-framework-part-1} and Table~\ref{table:compare-Freimut-with-framework-part-2}, we have effectively split Table~\ref{table:summary-of-framework} into two tables, adding brief meta-information into Table~\ref{table:compare-Freimut-with-framework-part-1}.

% Our mapping of the Freimut et al.~\cite{freimut05} article into the framework is clearly not exhaustive, and does not need to be. It is sufficient for Table~\ref{table:compare-Freimut-with-framework-part-1} and Table~\ref{table:compare-Freimut-with-framework-part-2} to show enough of a mapping to demonstrate that the Freimut et al.~\cite{freimut05} article and study recognise, even if only implicitly, enough elements of the framework. There are other excerpts from the Freimut et al.~\cite{freimut05} article we might report in the tables, and a given excerpt may be relevant to more than one element of the framework. Furthermore, a mapping of some part of the Freimut et al.~\cite{freimut05} study into the framework is not an indicator that Freimut et al.~\cite{freimut05} correctly addressed the respective element, only that they were aware of it and took action to address it. Finally, Freimut et al.~\cite{freimut05} may not have considered an element to the same level of abstraction that we have in the framework.

% The case study paper concerns the cost--effectiveness of software inspections. It was published in 2005 by Freimut et al.~\cite{freimut05}. The paper highlights that they carefully selected experts for the study. They used two selection criteria: professional role and experience. The three different roles were developers, testers and analysts. The experience of the individuals ranged from 3 to 18 years. It was noted that the responses differed based on the number of years of experience. Furthermore, the authors stress that having motivated experts is essential. This points to the fact that it may not be suitable to simply sample individuals based on some preset criteria. Finally, the authors also selected individuals that were currently doing the activity being researched. 

% The paper describes a number of essential aspects concerning participants in the case study. Given when the research was conducted, i.e., before 2005, the study was undertaken without the support of guidelines, at least from software engineering.

% In summary, the paper highlights four aspects related to the credibility of participants: role, experience, motivation and that the participants should currently perform the activity being researched. These aspects align with the framework.

% \begin{table*}[htp]
%     \small
%     \caption{Comparison of the Freimut et al.~\cite{freimut05} paper with framework}
%     \label{table:compare-Freimut-with-framework-part-1}
%     \centering
%     \begin{tabular}{| l |  p{11cm} | }
%         \toprule
%         \textbf{Criterion} & \textbf{Commentary}\\
%         \midrule
%         \multicolumn{2}{| l |}{\textbf{Meta-information about the study}}\\
%         Study type & Case study \\
%         Sample & 23 participants \\
%         Sampling & ``The QA management selected the experts following the rationale that they should be proactive and motivated developers and testers.''\\
%         \midrule
%         \multicolumn{2}{| l |}{\textbf{Information}}\\
%         Beliefs & Three types of expert estimate defect information\\
%         Facts & Collected from other sources, e.g., project data\\
%         \midrule
%         \multicolumn{2}{| l |}{\textbf{Quality criteria}}\\
%         Experience & ``The experts had various levels of experience in the business unit ranging from 3 to 18 years.'' \\
%         % Relevant & ``\dots an expert who is responsible for a very complex part of the system may provide estimates that are significantly different from other experts who are responsible for less complex system parts.''\\
%         Perception & \\
%         Selection & ``This question [of different scenarios] led the expert to think of `pathological' instances of defect corrections and their abnormally large associated effort. This had a significant impact on the practical maximum estimate.''\\
%         & ``One analyst mentioned in the interview that he had not participated in analysis inspections for a long time. Since his estimates about the correction effort of defects detected in analysis inspections differed from the other analysts, we decided to exclude this estimate.''\\
%         Reflection & ``\dots several experts were specifically asked whether they felt it was possible for them to estimate the required parameters. The pilot testers unanimously agreed that, with their experience, all parameters in our\dots models could be estimated, though, for some parameters (e.g., defect rework effort for defects introduced early but detected late), this might be a bit more difficult.''\\
%         Willingness & ``\dots experts were highly motivated during the interviews. They showed great interest in the study and the kind of questions they were asked.''\\
%         % & ``Very well received was the fact that the experts (i.e., the developers and testers) were involved in drawing conclusions about the inspection practices in the business unit. In some cases, the experts expressed their satisfaction and interest to the QA team. The experts were also very interested in receiving a copy of the final case study report to see the final results of their efforts.''\\
%         \midrule
%         \multicolumn{2}{| l |}{\textbf{Demographics}}\\
%         \multicolumn{2}{| l |}{Not reported}\\
%         \bottomrule
%     \end{tabular}
% \end{table*}       
 
% A case study is not directly comparable to interview studies and surveys because case studies incorporate more than one method of data collection. In Freimut et al.'s~\cite{freimut05} study, the researchers combine information provided by the participants with information collected as project data. The information provided by the experts is labeled as ``expert opinion'': for the framework, such information may be treated as beliefs, a type of information, provided by the participants.
      
%   \begin{table*}[htp]
%     \small
%     \caption{Comparison of the Freimut et al.~\cite{freimut05} paper with framework}
%     \label{table:compare-Freimut-with-framework-part-2}
%     \centering
%     \begin{tabular}{| l |  p{11cm} | }
%         \toprule
%         \textbf{Criterion} & \textbf{Commentary}\\   
%         \midrule
%         \multicolumn{2}{| l |}{\textbf{Falessi et al.~\cite{falessi2018empirical} R\textsuperscript{3} model}}\\
%         Real & ``The experts had various levels of experience in the business unit ranging from 3 to 18 years.'' \\
%         Relevant & ``\dots an expert who is responsible for a very complex part of the system may provide estimates that are significantly different from other experts who are responsible for less complex system parts.''\\
%         & ``Some of the experts with 3 to 4 years of experience had difficulties answering some of the questions regarding relatively rare events, such as the correction effort for analysis defects that are detected late in the system testing phase. Thus, experts should have a sufficient level of experience to be able to answer the questions. In a particular context, this should be determined during pilot testing.''\\
%         & ``However, two expert estimates show a significantly higher (practical) maximum value when compared to other experts. This might be due to the fact that all experts were responsible for different parts of the system.''\\
%         & ``\dots if that expert did not show relevant experience for the questions in the recent past or showed difficulties with the questions during the interview, then the answer was left out for the remainder of the analysis.''\\
%         Recent & ``In some cases, people who had worked a long time as developers, but were currently performing different tasks, provided estimates that differed significantly from the estimates of other experts.'' (p. 1090)\\
%         & ``One analyst mentioned in the interview that he had not participated in analysis inspections for a long time. Since his estimates about the correction effort of defects detected in analysis inspections differed from the other analysts, we decided to exclude this estimate.''\\
%         \midrule
%         \multicolumn{2}{| l |}{\textbf{Role}}\\
%         Performer & Analysts (n/16) estimate  correction cost for defects detected\\
%         & \hspace{3mm} in analysis inspections.\\
%         & ``\dots an expert who is currently not performing the task about which he is to provide an estimate may provide different estimates than an expert who is performing the task.''\\
%         & Testers (m/16) estimate effort for isolating faults from failures.\\
%         & Developers (7) estimate other effort \& defect information.\\
%         Observer & N/A\\
%         Advisor &  N/A\\
%         \bottomrule
%     \end{tabular}
% \end{table*}

% ``be estimated by one of three different roles in the development process: 1) Analysts, who can estimate the correction cost for defects detected in analysis inspections, 2) Testers, who can estimate the effort for isolating faults from failures, and 3) Developers, who can estimate effort and defects breakdowns for the remaining activities.'' (~\cite{freimut05}, p. 1085) 

% \subsection{OLD}

% The paper investigates practices in software maintenance, presenting four ``truths'' (Singer's term) about software maintenance, i.e., source code is the most important artefact; documentation is untrustworthy; organisations typically used some kind of maintenance control system, such as a bug-tracking database; and that if the problem can be reproduced, it can be solved.


% As an exemplar interview study, we selected a paper published by Singer \cite{singer1998practices} in 1998. This paper is published very `early', relative to most guidelines in software engineering. Thus, the paper does not use any (stated) guidelines when making research--design decisions.

% The paper focuses on practices in software maintenance. The main data collection method is interviews, however data was also collected in the form of project statistics. The study includes data from interviews of software maintenance practitioners from ten corporate groups. The interviews were conducted in pairs, to make the interviewees more comfortable. Furthermore, the interviewees were paired with a colleague having about the same level of experience in software maintenance.

% Interviewees were selected on the basis of them maintaining the current product for at least 12--18 months. This selection criterion helps ensure that the interviewees had both current and a certain amount of prior experience from maintaining a product. The interviews were tape recorded, and it was stressed that no manager should be able to identify even their particular organisation.

% The paper includes a good context description including application type, maintenance platform, programming language and general project statistics. Moreover, statistics concerning the participants are provided in the form of years of general experience, experience from the programming language used, knowledge of programming languages in general (number of languages) and time on the current project.

% In summary, the paper illustrates how practitioners are selected and paired based on their experience, including both general experience and current experience. Furthermore, the study ensures that the participants are comfortable through the pairing with individuals with similar experiences. The interview is well designed and conducted, and aligns with the framework, i.e., it does not provide any new aspect to be added to the framework.

% This highlights the difficulty of producing knowledge about the phenomenon of interest (in this case, UCD practice) from the information provided by participants, even a carefully selected set of participants.


% Vredenburg et al.'s~\cite{Vredenburg02} paper presents and discusses the \emph{respondent's} profiles and the \emph{UCD project} profiles. In other words, Vredenburg et al.'s~\cite{Vredenburg02} explicitly sought to assess the credibility of the respondents, although they do not explicitly talk in terms of credibility.

% A particularly interesting insight from the survey is the \emph{lack of consensus} from the respondents; respondents identified a total of 191 indicators of UCD effectiveness, and there there was little consensus. This highlights the difficulty of producing knowledge about the phenomenon of interest (in this case, UCD practice) from the information provided by participants, even a carefully selected set of participants.

% \subsection{OLD}

% As an exemplar survey study, we selected a paper published by Vredenburg et al.~\cite{Vredenburg02} in 2002. Vredenburg et al.~\cite{Vredenburg02} report a survey of user--centred design (UCD) practitioners. Their survey comprised over one hundred respondents drawn from the CHI'2000 attendees and the members of the Usability Professional Association (UPA).

% Vredenburg et al.~\cite{Vredenburg02} defined the target respondents as practitioners of UCD who had at least three years of experience with UCD, and who also considered UCD as their primary job. Vredenburg et al.~\cite{Vredenburg02} also asked respondents to the survey to consider a representative project. Vredenburg et al.~\cite{Vredenburg02} were therefore looking to recruit participants with Real, Relevant and Recent experience, as well as participants who were \emph{performers} in the situation of interest. 

% Vredenburg et al.'s~\cite{Vredenburg02} paper presents and discusses the \emph{respondent's} profiles and the \emph{UCD project} profiles. In other words, Vredenburg et al.'s~\cite{Vredenburg02} explicitly sought to assess the credibility of the respondents, although they do not explicitly talk in terms of credibility.

% A particularly interesting insight from the survey is the \emph{lack of consensus} from the respondents; respondents identified a total of 191 indicators of UCD effectiveness, and there there was little consensus. This highlights the difficulty of producing knowledge about the phenomenon of interest (in this case, UCD practice) from the information provided by participants, even a carefully selected set of participants.

% Overall, the paper provides a good example of recruiting participants with Real, Relevant and Recent experience (cf. Section \ref{subsubsection:roles}), of considering some demographics and of considering some of the additional characteristics, e.g., willingness, and quantity of situations experienced. Also two of the authors are themselves practitioners. 

==> x_notes.tex <==
\section*{Notes \& To Does}

\begin{enumerate}
    % \item Because this is a revision, we'll need to retain some kind of colour scheme to highlight changes for the reviewers. I suggest we settle on the colour \textcolor{blue}{blue} for the revisions we want to highlight to the reviewers. I realise that you (Claes) also uses \textcolor{blue}{blue}, and I think we can manage that. \claes{In this paper, I actually use a different colour, i.e., cyan.}
    \item We might use the concept of \emph{field study} and frame our work in terms of field studies. Lethbridge et al.~\cite{lethbridge2005studying} write,``Field study techniques are a group of methods that can be used individually or in combination to understand different aspects of real world environments.'' (\cite{lethbridge2005studying}, p. 312). The R3 and the framework both focus on real world environments. If we did so, we might update at least the following (these will look obvious - they're simply reminders):
    \begin{enumerate}
        \item The Title
        \item The Abstract 
        \item The Introduction \claes{Easily done in the Scope subsection}
        \item Other sections?
    \end{enumerate}
    
    \item Include Lenarduzzi et al.: Lenarduzzi  et al. has been added to Section~\ref{subsection:scope-of-article} and to Section~\ref{section:reviewingguidelines}.
    
    \item Define credibility somewhere in the paper, e.g., Introduction. Also, relate credibility to characteristics C1 - C5 in Table 1, as Reviewer 1 is asking about this.
    
    \item Considering adding functional roles to the framework.
    
    \item Clarify the distinction between factual information from participants and demographics.
    
    \item  Address point about ``pathological'' in Section 6 exemplars.
    
    \item To check that all Reviewers' Comments have been adequately responded to.
    
    \item AR to do an editorial review and revision of the Response to the Reviewers
    % \item I have retained Section \ref{section:review-guidelines} as a separate section at the moment, though moved it toward the front of the paper. My original suggestion, for the revised paper, was to incorporate Section \ref{section:review-guidelines} into related work. Section \ref{section:review-guidelines} \emph{might} be (significantly) distilled and if it is, it might naturally fit in Section \ref{section:related-work}. But if Section \ref{section:review-guidelines} remains a lengthier section it might be sensible to retain as a separate section. Also, I had thought of putting Section \ref{section:review-guidelines} toward the front of Section \ref{section:related-work}, but now I think Section \ref{section:review-guidelines} might better follow on from Section \ref{section:related-work}. I think these are two decisions to be made in due course, i.e.
    % \begin{enumerate}
    %     \item Whether to incorporate Section \ref{section:review-guidelines} into Section \ref{section:related-work} or keep separate; and
    %     \item If Section \ref{section:review-guidelines} is incorporated into Section \ref{section:related-work} where to incorporate it, e.g., toward the beginning.
    % \end{enumerate}
    % \item I was thinking that we might have a more-detailed worked example together with a high-level table summarising the three exemplars. So I started to apply the checklist to Curtis et al.'s~\cite{curtis1988field} ``A field study of the software design process for large systems''. Applying the checklist is raising some very interesting things\dots but doing so may be a lengthy digression from the current focus of the paper\dots I have paused that analyses for the moment.
    % \begin{enumerate}
    %     \item BUT one thing that is interesting is that Curtis et al. identify the concept of an \emph{exceptional designer} (alternatively titled, \emph{project guru}) who might be understood as \emph{key informant}.
    %     \item Freimut et al. also focus on expert opinion, which again might be understood as a kind of \emph{key informant}.
    % \end{enumerate}
    % \item I have also started to apply the checklist to the Freimut et al. paper, and I am finding a couple of things:
    % \begin{enumerate}
    %     \item There are ways in which the checklist might be tweaked; and
    %     \item Reflecting back, we used the three exemplars (if I recall correctly) to kind of `validate' the framework, e.g., the papers were corroborating our thinking. In a way, to then apply the checklist back to these three papers may be kind of circular. Possibly, we can say that the three papers both `validate' the framework and subsequently validate the checklist.
    % \end{enumerate}
    % \item Another option might be to simplify the framework and remove the checklist. These will save space that we can then use in a Section that goes into detail with the three exemplar papers.
    % \item The immediate `where nexts?' are:
    % \begin{enumerate}
    %     \item Work on Section~\ref{section:reference-examples} that applies the framework (and checklist) to the exemplar studies.
    %     \item Rework Section~\ref{section:related-work} and Section~\ref{section:review-guidelines} on related work
    %     \item Decide on the checklist: whether to have it, and what questions etc to have. \claes{Potentially the checklist may be submitted as supplementary material.}
    % \end{enumerate}
    
    
\end{enumerate}
